Probabilistic Label Trees for Extreme Multi-label Classification

Extreme multi-label classification (XMLC) is a learning task of tagging instances with a small subset of relevant labels chosen from an extremely large pool of possible labels. Problems of this scale can be efficiently handled by organizing labels as a tree, like in hierarchical softmax used for multi-class problems. In this paper, we thoroughly investigate probabilistic label trees (PLTs) which can be treated as a generalization of hierarchical softmax for multi-label problems. We first introduce the PLT model and discuss training and inference procedures and their computational costs. Next, we prove the consistency of PLTs for a wide spectrum of performance metrics. To this end, we upperbound their regret by a function of surrogate-loss regrets of node classifiers. Furthermore, we consider a problem of training PLTs in a fully online setting, without any prior knowledge of training instances, their features, or labels. In this case, both node classifiers and the tree structure are trained online. We prove a specific equivalence between the fully online algorithm and an algorithm with a tree structure given in advance. Finally, we discuss several implementations of PLTs and introduce a new one, napkinXC, which we empirically evaluate and compare with state-of-the-art algorithms.

==> 02-related.tex <==
\section{Related work}
\label{sec:related}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Some intro paragraph
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

We divide the related works by topic into label trees, extreme classification, and formal framework.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% label trees
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Label trees}

In a label tree~\citep{Bengio_et_al_2010} each label, or class in case of \multiclass{} classification, corresponds to one and only one path from the root to the leaf. The examples of \multiclass{} classification algorithms following this approach are filter trees~\citep{Beygelzimer_et_al_2009a,Li_Lin_2014} and probabilistic classifiers trees~\citep{Dembczynski_et_al_2016}. Similar algorithms were introduced independently in various fields: in deep networks, it is known as hierarchical softmax~\citep{Morin_Bengio_2005}, in statistics as nested dichotomies~\citep{Fox_1997}, and in multi-class regression as conditional probability  trees~\citep{Beygelzimer_et_al_2009b}. In pattern recognition a similar concept of multi-stage classifiers has also been considered~\citep{Kurzynski_1988}.

In extreme \multilabel{} classification this approach was applied in probabilistic label trees (\Algo{PLTs})~\citep{Jasinska_et_al_2016, Wydmuch_et_al_2018}.
A not probabilistic approach named Homer was introduced by~\citet{Tsoumakas_et_al_2008} to \multilabel, but not extreme, classification problems.
Other extreme \multilabel{} classification algorithms following the label tree approach were published as \Algo{Parabel}~\citep{Prabhu_et_al_2018}, \Algo{Bonsai Tree}~\citep{Babbar_Scholkopf_2019}, or \Algo{AttentionXML}~\citep{You_et_al_2019}.

A still open problem in label tree approaches is the tree structure learning.  
Conditional probability trees propose an online tree building method suited for \multiclass{} problems.
\Algo{fastText}~\citep{Joulin_et_al_2016} uses hierarchical softmax with a Huffman tree built on the label frequencies. 
\citet{Jernite_et_al_2017} have introduced a \Algo{Learned Tree} algorithm, which combines hierachical softmax with a hierarchical clustering that reassigns labels to paths in the tree in a semi-online manner. \Algo{Parabel} follows another approach in which a model similar to \Algo{PLT}s is trained in a batch mode and a tree is built by using recursively balanced k-means over the label profiles.
\citet{Busa-Fekete_et_al_2019} analyze the label tree building problem from the perspective of computational complexity of training and prediction.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% XMLC
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Extreme classification}

% The term \emph{extreme classification} was used by Manik Varma and John Langford to name their workshop organized at the \emph{Neural Information Processing Systems} (NIPS) conference in 2013. The workshop was a scientific response for many challenging applications characterized by very large output spaces. Extreme classification shed also new light on other machine learning problems. For example, raking or recommendation  can be reformulated into a multi-class or a multi-label task in which labels correspond to the ranked or recommended items. 

% Problems with a large number of classes used to be solved by nearest neighbor or decision tree methods. Some of recent algorithms are also based on these classical approaches, significantly extending them by a number of new tricks. If the number of classes is of order of thousands then an independent model for each class can be trained. This approach is usually named 1-vs-All approach. Unfortunately, 1-vs-All, when applied naively, scales linearly with the number of classes, which is too costly for many applications  

Extreme classification algorithms can be divided into several groups: embedding based, decision-tree based, smart 1-vs-All (or 1-vs-Rest), label-tree based, neural networks based, and others.
Embedding based methods reduce the original output space to a space with smaller dimensionality~\citep{Tai_Lin_2012} and build regression models in this low-dimensional space.
During classification of test examples, responses obtained in the low-dimensional space are transformed back to the original space.
The algorithms implementing that scheme differ in the compression and decompression methods. They use compressed sensing~\citep{Hsu_et_al_2009}, singular value decomposition~\citep{Tai_Lin_2012}, randomized principal component analysis~\citep{Mineiro_Karampatziakis_2015} or canonical correlation analysis in which the projection to the low dimensional space is combined with the transformation of the feature space~\citep{Chen_Lin_2012, Yu_et_al_2014}. \citet{Bhatia_et_al_2015} proposed sparse local embeddings (\Algo{SLEEC}) that use a k-nearest neighbor classifier in the embedding space to decompress the final prediction. This approach was further analyzed by \citet{Liu_Shen_2019}. \Algo{AnnexML}~\citep{Tagami_2017} uses a $k$-nearest neighbor graph of label vectors to perform efficient prediction in the embedding space.

%The second group consists of methods based on decision trees.
The direct use of standard decision tree algorithms can be very costly \citep{Agrawal_et_al_2013}. The \Algo{FastXML} algorithm~\citep{Prabhu_Varma_2014} reduces the cost of computation of splits of the feature space by use of linear classifiers in the  decision nodes. They are result of an alternating optimization of a multi-criteria objective. To improve accuracy, \Algo{FastXML} builds an ensemble of many trees. While \Algo{FastXML}, as a majority of decision tree algorithms, works in a batch mode,  \citet{Choromanska_Langford_2015} introduced an online decision tree algorithm that also uses linear classifiers in the internal nodes of the tree. The idea of \Algo{FastXML} is followed by \Algo{PfastreXML}~\citep{Jain_et_al_2016}, which optimizes propensity scored variants of performance metrics, and \Algo{CraftML}~\citep{Siblini_et_al_2018}, which increases randomness in building the ensemble of trees, and uses random projections and k-means clustering to create the decision nodes classifiers.
\citet{Liu_Tsang_2017} propose different variant of decision trees suited for large output spaces, building a structure of label sets, for which they provide theoretical analysis, sometimes missing in XMLC papers.
Recently, \citet{Majzoubi_Choromanska_2019} proposed \Algo{LdSM}, building decision-tree node by node by streaming observations multiple times, and optimizing an objective joining class purity of children nodes, balancedness and number of child nodes where a single observation ends up.

In label tree based algorithms each label corresponds to one and only one path from the tree root to a leaf, and classifiers correspond to tree nodes. To predict multiple labels, multiple leafs should be selected. 
%\Algo{HOMER}~\citep{Tsoumakas_et_al_2008} applied this approach to \multilabel problems, using classifiers delivering binary predictions in the tree nodes.
Probabilistic label trees~\citep{Jasinska_et_al_2016, Wydmuch_et_al_2018} applied the label tree approach to XMLC.
%Contrary to \Algo{HOMER}, they use probabilistic classifiers in the tree ones. 
Other XMLC algorithms following the label tree approach were published as \Algo{Parabel}~\citep{Prabhu_et_al_2018}, \Algo{Bonsai Tree}~\citep{Babbar_Scholkopf_2019}, or \Algo{AttentionXML}~\citep{You_et_al_2019}.

The smart 1-vs-All approaches train a single binary classifier per label, but reduce the computational cost of such method compared to naive implementation by use of distributed computation and weight pruning (\Algo{DiSMEC},~\citet{Babbar_Scholkopf_2017}), 
exploring different optimization and prediction methods (\Algo{PD-Sparse},~\citet{Yen_et_al_2016}; \Algo{PPD-Sparse},~\citet{Yen_et_al_2017}),
or both (\Algo{ProXML},~\citet{Babbar_Scholkopf_2019}). \citet{Bamler_et_al_2020} use a hierarchical softmax based negative sampling to efficiently train a single classifier per label, however their approach seems to underperform compared to other XMLC algorithms.

The algorithms that do not fit any of those groups, but are not deep learning based, propose various methods for efficient handling of large label spaces, by avoiding a linear scan over all labels. \citet{Niculescu-Mizil_Abbasnejad_2015} propose label filters that use projections to select candidate labels, while \citet{Cisse_et_al_2013} use Bloom filters. Recently, \citet{Medini_et_al_2019} used universal hashing to perform extreme \multiclass{} classification in memory logarithmic to the number of labels. \Algo{LTLS}~\citep{Jasinska_Karampatziakis_2017} and \Algo{Wide-LTLS}~\citep{Evron_et_al_2018} use classifiers structured as a graph and Viterbi algorithm for inference to perform extreme \multiclass{} classification in both time and space logarithmic in number of labels.

The already mentioned hierarchical softmax is often used as an output layer in neural networks. The \Algo{fastText} implementation, or the \Algo{extremeText}~\citep{Wydmuch_et_al_2018}, can also be viewed as a shallow architecture with one hidden layer that represents instances as averaged feature (i.e., word) vectors. 
Another neural network-based model designed for XMLC has been introduced in~\citep{Liu_et_al_2017}. This model, referred to as \Algo{XML-CNN}, uses a complex convolutional deep network with a narrow last layer to make it work with large output spaces.
\Algo{AttentionXM}L~\citep{You_et_al_2019} uses a label tree to efficiently produce output of a \Algo{BiLSTM} model with a \multilabel{} attention.
\Algo{X-BERT}~\citep{Chang_et_al_2019} uses a modified \Algo{BERT}~\citep{bert} model to predict meta-label, and then uses 1-vs-All model, evaluated only for labels included in the meta-label, to rank the subset of labels.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% other...
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Learning reductions and formal framework}

The theoretical analysis of predictive performance of extreme classification methods can be performed within statistical learning theory~\citep{Devroye_et_al_1998,Hastie_et_al_2003}, the learning reductions framework (reduction to simple learning problems)~\citep{Beygelzimer_et_al_2008} or online learning~\citep{Cesa-Bianchi_Lugosi_2006}. The main objective of the theoretical analysis is to find statistical guarantees for the error rate that do not depend on the total number of labels or this dependence is strongly sublinear. In the former case, the bound can be expressed, for example, by the average number of positive labels (which is certainly much less than the total number of labels). %It is noteworthy that the theoretical theoretical strongly depends on a chosen performance measure.
Some first results of this type has already been obtained in terms of statistical learning theory, for example, in~\citep{Bhatia_et_al_2015, Lei_et_al_2016}. Also in the framework of learning reductions, promising results have been published~\citep{Beygelzimer_et_al_2009a, Beygelzimer_et_al_2009b, Dembczynski_et_al_2016, Jasinska_et_al_2016}, which relate the performance of the extreme classification problem to the performance of a series of derived, simple classification tasks such as binary classification. 
\citet{Liu_Tsang_2017} analyze the generalization error of their proposed approach.
\citet{Majzoubi_Choromanska_2019} use boosting theory to analyze the quality of predictions obtained using tree with multiple splits.

%#Interestingly, it seems that so far no direct analysis of extreme classification methods has been conducted in the context of online learning. 



==> headers.tex <==

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts

% I like coloured links, but jmlr loading makes a clash if this is loaded
%\usepackage{hyperref}       % hyperlinks
%\hypersetup{colorlinks,linkcolor={blue},citecolor={blue},urlcolor={black}} 
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography

\usepackage{afterpage}
\usepackage{subcaption} 

\usepackage{amssymb,amsthm,amsmath}
%\usepackage[numbers]{natbib}
\usepackage{array,graphicx}
\usepackage{comment}
\usepackage{wrapfig}

% Attempt to make hyperref and algorithmic work together better:
\newcommand{\theHalgorithm}{\arabic{algorithm}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{amsmath} 
\usepackage{amssymb} 

% without those there is an error loading jmlr style
\let\proof\relax 
\let\endproof\relax

\usepackage{amsthm}
\usepackage{mathtools} 
\usepackage{stmaryrd}
\usepackage{bm}
\usepackage{tikz}
\usetikzlibrary{calc}
\usetikzlibrary{decorations}
\usepackage{longtable}
\usepackage{multirow}
\usepackage{makecell}

\usepackage{thmtools, thm-restate}
%\setlength\tabcolsep{2pt}
%\usepackage[subtle,mathspacing=normal, tracking=normal]{savetrees}
%\usepackage{microtype}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% TIKZ plots
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{tikz}
% \usepackage{fancybox}
% \usepackage{amssymb} 
% \usepackage{amsthm}
% \usepackage{stmaryrd}
\usepackage{pgfplots}
\usetikzlibrary{arrows}
% \usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{positioning}
\usetikzlibrary{decorations.text}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.shapes}
% \usetikzlibrary{shapes,snakes}

\usetikzlibrary{pgfplots.groupplots}
\usepgfplotslibrary{fillbetween}
\usetikzlibrary{patterns}
%\usepgfplotslibrary{groupplots}

\usepackage{lscape}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Command
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% OPLT
\definecolor{myteal}{HTML}{2380D8}
\definecolor{myred}{HTML}{EA2222}
\definecolor{mypurple}{HTML}{9900CC}
\definecolor{mygrey}{HTML}{494949}
\definecolor{mygreen}{HTML}{008000}
\definecolor{myblack}{HTML}{000000}
\definecolor{mywhite}{HTML}{FFFFFF}
%\definecolor{putblue}{RGB}{0,96,124}
\definecolor{yahooviolet}{RGB}{66, 2, 176}
\definecolor{putblue}{RGB}{0, 103, 144}
\definecolor{allegroorange}{RGB}{255, 90, 0}
\definecolor{putred}{RGB}{204,33,69}

\usepackage{adjustbox}

\makeatletter

\newcommand*{\eifstartswith}{\@expandtwoargs\ifstartswith}
\newcommand*{\ifstartswith}[2]{%
  \if\@car#1.\@nil\@car#2.\@nil
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\Algo}[1]{\textsc{#1}}
\newcommand{\Algo}[1]{\textsc{#1}}

\renewcommand{\vec}[1]{\boldsymbol{#1}}

\newcommand{\bx}{\vec{x}}
\newcommand{\by}{\vec{y}}
\newcommand{\bz}{\vec{z}}
\newcommand{\bw}{\vec{w}}
\newcommand{\bh}{\vec{h}}
\newcommand{\bc}{\vec{c}}
\newcommand{\balpha}{\vec{\alpha}}
\newcommand{\btheta}{\vec{\theta}}
\newcommand{\btau}{\vec{\tau}}
\newcommand{\bX}{\vec{X}}
\newcommand{\bY}{\vec{Y}}


\newcommand{\bzt}{\vec{z}_{t}}
\newcommand{\ztlt}{z_{t,l_t}}
\newcommand{\bztltmone}{\vec{z}_{t}^{l_t-1}}


\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calLp}{\mathcal{L_{+}}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calW}{\mathcal{W}}

\newcommand{\dataset}{{\cal D}}

\newcommand{\etanode}{\eta^n}

\newcommand{\fracpartial}[2]{\frac{\partial #1}{\partial  #2}}

\newcommand{\heta}{\hat{\eta}}
\newcommand{\hy}{\hat{y}}
\newcommand{\hetanode}{\hat{\eta}^n}

\newcommand\E{\mathbb{E}}   % for the real numbers
\newcommand\R{\mathbb{R}}   % for the real numbers
\newcommand\N{\mathbb{N}}   % for the natural numbers

\newcommand{\pa}[1]{\mathrm{pa}(#1)}
\newcommand{\leaf}[1]{\textrm{leaf}(#1)}
\newcommand{\Path}[1]{\mathrm{Path}(#1)}
\newcommand{\lenpath}{\mathrm{len}}
\newcommand{\depth}{\mathrm{depth}}

\newcommand{\precat}[1]{precision$@#1$}
\newcommand{\Precat}[1]{Precision$@#1$}
\newcommand{\precatk}{precision$@k${}}
\newcommand{\Precatk}{Precision$@k${}}
\newcommand{\psimacro}{$\Psi_{\mathrm{macro}(\bx)}$ }
\newcommand{\psimicro}{$\Psi_{\mathrm{micro}(\bx)}$ }

\newcommand{\prob}{\mathbf{P}} 
\newcommand{\hprob}{\widehat\prob}
\newcommand{\reg}{\mathrm{reg}}
\newcommand{\regret}{\mathrm{Reg}}
\newcommand{\risk}{\mathrm{Risk}}
\newcommand{\riskcond}{\mathrm{risk}}
\newcommand{\loss}{R}

\newcommand{\lossfunc}{\ell}

\newcommand{\lonemarginalserror}{$|\eta_j(\bx) - \hat{\eta}_j(\bx)|$}

\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{a}}
%\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}

\newcommand{\mM}{\boldsymbol{M}}
\newcommand{\mW}{\boldsymbol{W}}


% For complexity
\newcommand{\ct}{\mathrm{c_T}}
\newcommand{\cp}{\mathrm{c_P}}
\newcommand{\CT}{\mathrm{C_T}}
\newcommand{\CP}{\mathrm{C_P}}
\newcommand{\internalsubtree}{\mathrm{S}}
\newcommand{\internalfull}{\mathrm{internal}}
\newcommand{\internal}{\mathcal{I}}
\newcommand{\leavest}{\mathcal{L}_t}
% \newcommand{\leaves}{\mathcal{L}}


\newcommand{\parent}{\mathrm{pa}}
\newcommand{\childs}[1]{\mathrm{Ch}(#1)}
\newcommand{\children}{\mathrm{ch}}

%tree definition
\renewcommand{\root}{r}
\newcommand{\nodes}{V}
\newcommand{\vertices}{V}
\newcommand{\tree}{T}
\newcommand{\leaves}{L}
\newcommand{\leafnode}{l}
\newcommand{\labels}{\calL}
\newcommand{\vertex}{v}
\newcommand{\node}{v}

% codes definition
\newcommand{\vertexcode}{\bz_{v}}
\newcommand{\vertexcodelen}{d_{\bz_{v}}}
%\newcommand{\vertexcodelen}{|\bz_{v}|}
\newcommand{\vertexcodeelem}[1]{z_{v, #1}}
\newcommand{\vertexcodeprefix}[1]{\bz_{v}^{#1}}

\newcommand{\lblcode}{\bz_{j}}
% \newcommand{\lblcodelen}{|\bz_{j}|}
\newcommand{\lblcodelen}{d_{\bz_{j}}}
\newcommand{\lblcodeelem}[1]{z_{j, #1}}
\newcommand{\lblcodeprefix}[1]{\bz_{j}^{#1}}

\newcommand{\code}{\bz}
% \newcommand{\codelen}{|\bz|}
\newcommand{\codelen}{d_{\bz}}
\newcommand{\codelenj}{d_{\bz_{j}}}
\newcommand{\codeelem}[1]{z_{#1}}
\newcommand{\codeprefix}[1]{\bz^{#1}}
\newcommand{\codelenshort}{d}



\newcommand{\encode}{\sigma}
\newcommand{\decode}{\sigma^{-1}}

\newcommand{\plt}{\Algo{PLT} }
\newcommand{\plts}{\Algo{PLTs} }

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % codes definition for test
% \newcommand{\vertexcode}{\mathbf{a}_{v}}
% \newcommand{\vertexcodelen}{|\mathbf{a}_{v}|}
% \newcommand{\vertexcodeelem}[1]{a_{v, #1}}
% \newcommand{\vertexcodeprefix}[1]{\mathbf{a}_{v}^{#1}}

% \newcommand{\lbljcode}{\mathbf{a}_{j}}
% \newcommand{\lbljcodelen}{|\mathbf{a}_{j}|}
% \newcommand{\lbljcodeelem}[1]{a_{j, #1}}
% \newcommand{\lbljcodeprefix}[1]{\mathbf{a}_{j}^{#1}}

% \newcommand{\lblcode}{\mathbf{a}}
% \newcommand{\lblcodelen}{|\mathbf{a}|}
% \newcommand{\lblcodeelem}[1]{a_{#1}}
% \newcommand{\lblcodeprefix}[1]{\mathbf{a}^{#1}}
% \newcommand{\lblcodelenshort}{c}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% generalized classif perf metrics
\newcommand{\FP}{\mathrm{FP}}
\newcommand{\FN}{\mathrm{FN}}
\newcommand{\TP}{\mathrm{TP}}
\newcommand{\TN}{\mathrm{TN}}

% how we write things
%\newcommand{\plt}{\Algo{PLT} }
%\newcommand{\plts}{\Algo{PLTs} }
\newcommand{\multilabel}{multi-label}
\newcommand{\multiclass}{multi-class}

\newcommand{\eurlex}{EurLex-4K}
\newcommand{\amazoncatsmall}{AmazonCat-13K}
\newcommand{\amazoncatlarge}{AmazonCat-14K}
\newcommand{\wikiten}{Wiki10-30K}
\newcommand{\deliciouslarge}{DeliciousLarge-200K}
\newcommand{\wikilshtc}{WikiLSHTC-325K}
\newcommand{\wikipedia}{WikipediaLarge-500K}
\newcommand{\amazon}{Amazon-670K}
\newcommand{\amazonlarge}{Amazon-3M}

%%%%%%%%%%%%%%%%%
% for pseudocodes


\algnewcommand{\IIf}[1]{\State\algorithmicif\ #1\ \algorithmicthen}
\algnewcommand{\IElse}[1]{\State\algorithmicelse\ #1\ }
\algnewcommand{\IElseIf}[1]{\State\algorithmicelse \algorithmicif\ #1\  \algorithmicthen}
\algnewcommand{\EndIIf}{\unskip\ \algorithmicend\ \algorithmicif}
\algnewcommand{\IfThen}[2]{\State\algorithmicif\ #1\ \algorithmicthen\ #2\ }
\algnewcommand{\ForDo}[2]{\State\algorithmicfor\ #1\ \algorithmicdo\ #2\ }


\newcommand{\Func}[1]{\mathrm{#1}}
\newcommand{\HLFunc}[1]{\mathrm{\textbf{#1}}}
\newcommand{\hby}{\hat{\by}}
%%%%%%%%%%%%%%%%

\newcommand\todo[1]{\textcolor{magenta}{#1}}


\newcommand{\datasix}[6]{
    \begin{tabular}{ll}
    \rule{0pt}{0pt} #1 \\
    \rule{0pt}{0pt} #2 \\
    \rule{0pt}{0pt} #3 \\
    \rule{0pt}{0pt} #4 \\
    \rule{0pt}{0pt} #5 \\
    \rule{0pt}{0pt} #6 \\
    \end{tabular}
}

\newcommand{\datafive}[5]{
    \begin{tabular}{ll}
    \rule{0pt}{0pt} #1 \\
    \rule{0pt}{0pt} #2 \\
    \rule{0pt}{0pt} #3 \\
    \rule{0pt}{0pt} #4 \\
    \rule{0pt}{0pt} #5 \\
    \end{tabular}
}

\newcommand{\datafour}[4]{
    \begin{tabular}{ll}
    \rule{0pt}{0pt} #1 \\
    \rule{0pt}{0pt} #2 \\
    \rule{0pt}{0pt} #3 \\
    \rule{0pt}{0pt} #4 \\
    \end{tabular}
}

\newcommand{\data}[3]{
    \begin{tabular}{ll}
    \rule{0pt}{0pt} #1 \\
    \rule{0pt}{0pt} #2 \\
    \rule{0pt}{0pt} #3 \\
    \end{tabular}
}

\newcommand{\datatwo}[3]{
    \begin{tabular}{cc}
    \rule{0pt}{0pt} #1 \\
    \rule{0pt}{0pt} #2 \\
    \end{tabular}
}


\newcommand{\databf}[3]{
    \textbf{
	\begin{tabular}{ll}
    \rule{0pt}{0pt} #1 \\
    \rule{0pt}{0pt} #2 \\
    \rule{0pt}{0pt} #3 \\
    \end{tabular}
	}
}

\newcommand{\datall}[2]{
    \begin{tabular}{ll}
    \rule{0pt}{0pt} #1 \\
    \rule{0pt}{0pt} #2 \\
    \end{tabular}
}


\newcommand{\datarr}[2]{
    \begin{tabular}{rr}
    \rule{0pt}{0pt} #1 \\
    \rule{0pt}{0pt} #2 \\
    \end{tabular}
}


\newcommand{\assert}[1]{\llbracket #1 \rrbracket}

\newcommand{\given}{\, | \,}

\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}

\DeclareMathOperator*{\argmax}{\arg \max}
\DeclareMathOperator*{\argmin}{\arg \min}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% spaces
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\figureWidthTwo}{0.6\textwidth}

\newcommand{\figureBetween}{0pt}
\newcommand{\figureBetweenHorizontal}{0pt}

\newcommand{\sectionBefore}{-0pt}
\newcommand{\sectionAfter}{-0pt}

\newcommand{\tableBefore}{-0pt}
\newcommand{\tableAfter}{-0pt}

\newcommand{\figureBefore}{-0pt}
\newcommand{\figureAfter}{-0pt}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\figures}{./Figs}


==> ncn.tex <==

\acks{The work of Kalina Jasinska-Kobus was supported by the Polish National Science Center under grant 
no.~2017/25/N/ST6/00747. Computational experiments have been performed in Poznan Supercomputing and Networking Center.
}
%This research has been partially supported by the statutory funds of Poznan University of Technology

==> notation.tex <==


$\precatk$

% $$
% \eta_j(\bx) = \prob(\bz \given \bx) = \prod_{i=1}^l \prob(z_i \given \bz^{i-1}, \bx) 
% $$

% $$
% \heta_j(\bx) = \hprob(\bz \given \bx) = \prod_{i=1}^l \hprob(z_i \given \bz^{i-1}, \bx)
% $$

% $$
% \etanode_t(\bx) = \prob(\bz_t \given \bx) = \prod_{i=1}^{l_t} \prob(z_{t,i} \given \bzt^{i-1}, \bx) 
% $$

% $$
% \hetanode_t(\bx) = \hprob(\bz_t \given \bx) = \prod_{i=1}^{l_t} \hprob(z_{t,i} \given \bzt^{i-1}, \bx) 
% $$

% $\vertices$ -- all nodes in tree $\tree$ -- all codes?


$j \in \labels$

$\labels = \{1, 2, \ldots, m\}$

$v \in \vertices$ any tree node

$\vertices$ -- the set of the vertices in $\tree$

$\tree_v$ -- the subtree of $\tree$ rooted in node $v$

$L_v$ -- the labels assigned to leaf nodes of the subtree of $\tree$ rooted in node $v$

$\leafnode_j$ - the leaf corresponding to label $j$

$\leafnode_j \in \leaves$

$\vertices \setminus \leaves$ -- internal nodes

$t$ nodes in the tree $\tree$

$\eta_v(\bx)$

$\eta_{\leafnode_j}(\bx) = \eta_j(\bx)$

$\lblcode$ corresponds to node $v$

If not stated differently, code $\lblcode$ corresponds to the leaf node $\leafnode_j$

$$
\eta_v(\bx) = \prob(\bz \given \bx) = \prod_{i=1}^{\lblcodelen} \prob(\lblcodeelem{i} \given \lblcodeprefix{i-1}, \bx) 
$$

with $\lblcodelen$ we denote the length of the code $\lblcode$

\todo{sprawdzic czy to odpowiada definicji l wczesniej uzywanej}

\todo{czy to nie powinno byc od zera?}

$$
\heta_v(\bx) = \hprob(\lblcode \given \bx) = \prod_{i=1}^{\lblcodelen} \hprob(\lblcodeelem{i} \given \lblcodeprefix{i-1}, \bx) 
$$

$$
\eta_{\leafnode_j}(\bx) = \eta_j(\bx)
$$

$$
\heta_{\leafnode_j}(\bx) = \heta_j(\bx)
$$





==> pp.tex <==



==> tables/table-plt-vs-sota.tex <==


\begin{center}
\footnotesize
\begin{longtable}[h]{l|r@{}lr@{}lr@{}l|r@{}lr@{}lr@{}l}

\specialrule{0.94pt}{0.4ex}{0.65ex}
\multicolumn{13}{c}{\textbf{\eurlex}} \\
\multicolumn{1}{c|}{} & \multicolumn{2}{c}{$p@1$ [\%]} & \multicolumn{2}{c}{$p@3$ [\%]} & \multicolumn{2}{c|}{$p@5$ [\%]} 
& \multicolumn{2}{c}{$T_{\textrm{train}}$ [h]} & \multicolumn{2}{c}{$T/N_{\textrm{test}}$ [ms]} & \multicolumn{2}{c}{$M_{\textrm{size}}$ [GB]} \\
\midrule
\Algo{FastXML} & $71.26$ & $\pm 0.19$ & $59.80$ & $\pm 0.12$ & $50.28$ & $\pm 0.02$ & $0.07$ & $\pm 0.00$ & $0.97$ & $\pm 0.15$ & $0.22$ & $\pm 0.00$ \\
\Algo{PfastreXML} & $70.21$ & $\pm 0.09$ & $59.26$ & $\pm 0.10$ & $50.59$ & $\pm 0.08$ & $0.08$ & $\pm 0.00$ & $1.30$ & $\pm 0.09$ & $0.26$ & $\pm 0.00$ \\
\Algo{PPDSparse} & \multicolumn{2}{c}{$83.83$} & \multicolumn{2}{c}{$70.72$} & \multicolumn{2}{c|}{$59.21$} & \multicolumn{2}{c}{$0.02$} & \multicolumn{2}{c}{$1.00$} & \multicolumn{2}{c}{$0.07$} \\
\Algo{DiSMEC} & \multicolumn{2}{c}{$83.67$} & \multicolumn{2}{c}{$70.70$} & \multicolumn{2}{c|}{$59.14$} & \multicolumn{2}{c}{$0.08$} & \multicolumn{2}{c}{$7.00$} & \multicolumn{2}{c}{$0.04$} \\

\midrule
\Algo{Parabel-T=1} & $80.66$ & $\pm 0.16$ & $67.76$ & $\pm 0.05$ & $56.57$ & $\pm 0.07$ & $0.01$ & $\pm 0.00$ & $0.25$ & $\pm 0.00$ & $0.01$ & $\pm 0.00$ \\
\Algo{Parabel-T=3} & $81.80$ & $\pm 0.10$ & $68.67$ & $\pm 0.03$ & $57.45$ & $\pm 0.06$ & $0.02$ & $\pm 0.00$ & $0.93$ & $\pm 0.04$ & $0.03$ & $\pm 0.00$ \\
\Algo{XT-T=1} & $77.29$ & $\pm 0.21$ & $64.41$ & $\pm 0.11$ & $53.56$ & $\pm 0.11$ & $0.21$ & $\pm 0.00$ & $0.36$ & $\pm 0.00$ & $0.02$ & $\pm 0.00$ \\
\Algo{XT-T=3} & $78.66$ & $\pm 0.13$ & $65.48$ & $\pm 0.16$ & $54.63$ & $\pm 0.05$ & $0.36$ & $\pm 0.02$ & $0.98$ & $\pm 0.02$ & $0.03$ & $\pm 0.00$ \\
\Algo{PLT-T=1} & $80.51$ & $\pm 0.16$ & $65.65$ & $\pm 0.40$ & $53.33$ & $\pm 0.68$ & $0.02$ & $\pm 0.00$ & $0.39$ & $\pm 0.03$ & $0.02$ & $\pm 0.00$ \\
\Algo{PLT-T=3} & $81.39$ & $\pm 0.13$ & $67.49$ & $\pm 0.31$ & $55.65$ & $\pm 0.47$ & $0.04$ & $\pm 0.00$ & $1.33$ & $\pm 0.07$ & $0.06$ & $\pm 0.00$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}
\multicolumn{13}{c}{\textbf{\amazoncatsmall}} \\
\multicolumn{1}{c|}{} & \multicolumn{2}{c}{$p@1$ [\%]} & \multicolumn{2}{c}{$p@3$ [\%]} & \multicolumn{2}{c|}{$p@5$ [\%]} 
& \multicolumn{2}{c}{$T_{\textrm{train}}$ [h]} & \multicolumn{2}{c}{$T/N_{\textrm{test}}$ [ms]} & \multicolumn{2}{c}{$M_{\textrm{size}}$ [GB]} \\
\midrule
\Algo{FastXML} & $93.03$ & $\pm 0.00$ & $78.22$ & $\pm 0.01$ & $63.38$ & $\pm 0.00$ & $5.53$ & $\pm 0.15$ & $1.06$ & $\pm 0.08$ & $18.35$ & $\pm 0.00$ \\
\Algo{PfastreXML} & $85.62$ & $\pm 0.01$ & $75.31$ & $\pm 0.00$ & $62.83$ & $\pm 0.01$ & $5.45$ & $\pm 0.12$ & $0.98$ & $\pm 0.06$ & $19.01$ & $\pm 0.00$ \\
\Algo{PPDSparse} & \multicolumn{2}{c}{$92.72$} & \multicolumn{2}{c}{$78.14$} & \multicolumn{2}{c|}{$63.41$} & \multicolumn{2}{c}{$0.00$} & \multicolumn{2}{c}{$0.00$} & \multicolumn{2}{c}{$0.00$} \\
\Algo{DiSMEC} & \multicolumn{2}{c}{$92.72$} & \multicolumn{2}{c}{$78.11$} & \multicolumn{2}{c|}{$63.40$} & \multicolumn{2}{c}{$0.00$} & \multicolumn{2}{c}{$0.00$} & \multicolumn{2}{c}{$0.00$} \\

\midrule
\Algo{Parabel-T=1} & $92.58$ & $\pm 0.02$ & $78.53$ & $\pm 0.00$ & $63.90$ & $\pm 0.01$ & $0.19$ & $\pm 0.00$ & $0.22$ & $\pm 0.00$ & $0.21$ & $\pm 0.00$ \\
\Algo{Parabel-T=3} & $93.24$ & $\pm 0.01$ & $79.17$ & $\pm 0.00$ & $64.51$ & $\pm 0.00$ & $0.64$ & $\pm 0.03$ & $1.05$ & $\pm 0.04$ & $0.62$ & $\pm 0.00$ \\
\Algo{XT-T=1} & $91.96$ & $\pm 0.02$ & $77.41$ & $\pm 0.01$ & $62.75$ & $\pm 0.02$ & $10.75$ & $\pm 0.71$ & $0.17$ & $\pm 0.01$ & $0.41$ & $\pm 0.00$ \\
\Algo{XT-T=3} & $92.47$ & $\pm 0.02$ & $78.13$ & $\pm 0.02$ & $63.44$ & $\pm 0.02$ & $24.38$ & $\pm 1.06$ & $0.56$ & $\pm 0.01$ & $0.46$ & $\pm 0.00$ \\
\Algo{PLT-T=1} & $93.04$ & $\pm 0.02$ & $78.44$ & $\pm 0.02$ & $63.70$ & $\pm 0.02$ & $0.72$ & $\pm 0.02$ & $0.32$ & $\pm 0.03$ & $0.35$ & $\pm 0.00$ \\
\Algo{PLT-T=3} & $93.30$ & $\pm 0.04$ & $78.89$ & $\pm 0.05$ & $64.12$ & $\pm 0.05$ & $1.80$ & $\pm 0.06$ & $0.81$ & $\pm 0.03$ & $1.06$ & $\pm 0.00$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}
\multicolumn{13}{c}{\textbf{\wikiten}} \\
\multicolumn{1}{c|}{} & \multicolumn{2}{c}{$p@1$ [\%]} & \multicolumn{2}{c}{$p@3$ [\%]} & \multicolumn{2}{c|}{$p@5$ [\%]} 
& \multicolumn{2}{c}{$T_{\textrm{train}}$ [h]} & \multicolumn{2}{c}{$T/N_{\textrm{test}}$ [ms]} & \multicolumn{2}{c}{$M_{\textrm{size}}$ [GB]} \\
\midrule
\Algo{FastXML} & $82.97$ & $\pm 0.02$ & $67.58$ & $\pm 0.07$ & $57.68$ & $\pm 0.03$ & $0.23$ & $\pm 0.01$ & $8.21$ & $\pm 0.52$ & $0.54$ & $\pm 0.00$ \\
\Algo{PfastreXML} & $75.58$ & $\pm 0.07$ & $64.38$ & $\pm 0.11$ & $57.25$ & $\pm 0.07$ & $0.23$ & $\pm 0.00$ & $10.40$ & $\pm 0.41$ & $1.13$ & $\pm 0.00$ \\
\Algo{PPDSparse} & \multicolumn{2}{c}{$73.80$} & \multicolumn{2}{c}{$60.90$} & \multicolumn{2}{c|}{$50.40$} & \multicolumn{2}{c}{$0.00$} & \multicolumn{2}{c}{$0.00$} & \multicolumn{2}{c}{$0.00$} \\
\Algo{DiSMEC} & \multicolumn{2}{c}{$85.20$} & \multicolumn{2}{c}{$74.60$} & \multicolumn{2}{c|}{$65.90$} & \multicolumn{2}{c}{$0.00$} & \multicolumn{2}{c}{$0.00$} & \multicolumn{2}{c}{$0.00$} \\

\midrule
\Algo{Parabel-T=1} & $84.17$ & $\pm 0.03$ & $72.12$ & $\pm 0.04$ & $63.30$ & $\pm 0.05$ & $0.07$ & $\pm 0.00$ & $0.86$ & $\pm 0.02$ & $0.06$ & $\pm 0.00$ \\
\Algo{Parabel-T=3} & $84.49$ & $\pm 0.05$ & $72.57$ & $\pm 0.04$ & $63.66$ & $\pm 0.10$ & $0.20$ & $\pm 0.00$ & $2.67$ & $\pm 0.06$ & $0.18$ & $\pm 0.00$ \\
\Algo{XT-T=1} & $85.76$ & $\pm 0.06$ & $74.37$ & $\pm 0.10$ & $64.44$ & $\pm 0.05$ & $0.72$ & $\pm 0.06$ & $0.91$ & $\pm 0.06$ & $0.25$ & $\pm 0.00$ \\
\Algo{XT-T=3} & $85.41$ & $\pm 0.14$ & $74.49$ & $\pm 0.07$ & $64.70$ & $\pm 0.11$ & $1.55$ & $\pm 0.04$ & $1.78$ & $\pm 0.07$ & $0.37$ & $\pm 0.00$ \\
\Algo{PLT-T=1} & $85.36$ & $\pm 0.09$ & $73.90$ & $\pm 0.07$ & $63.84$ & $\pm 0.07$ & $0.21$ & $\pm 0.00$ & $5.35$ & $\pm 0.32$ & $0.58$ & $\pm 0.00$ \\
\Algo{PLT-T=3} & $85.55$ & $\pm 0.05$ & $74.39$ & $\pm 0.10$ & $64.41$ & $\pm 0.07$ & $0.55$ & $\pm 0.02$ & $17.92$ & $\pm 0.56$ & $1.75$ & $\pm 0.00$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}
\multicolumn{13}{c}{\textbf{\deliciouslarge}} \\
\multicolumn{1}{c|}{} & \multicolumn{2}{c}{$p@1$ [\%]} & \multicolumn{2}{c}{$p@3$ [\%]} & \multicolumn{2}{c|}{$p@5$ [\%]} 
& \multicolumn{2}{c}{$T_{\textrm{train}}$ [h]} & \multicolumn{2}{c}{$T/N_{\textrm{test}}$ [ms]} & \multicolumn{2}{c}{$M_{\textrm{size}}$ [GB]} \\
\midrule
\Algo{FastXML} & $43.17$ & $\pm 0.03$ & $38.70$ & $\pm 0.01$ & $36.22$ & $\pm 0.02$ & $3.86$ & $\pm 0.09$ & $12.27$ & $\pm 0.36$ & $6.95$ & $\pm 0.00$ \\
\Algo{PfastreXML} & $17.44$ & $\pm 0.02$ & $17.28$ & $\pm 0.01$ & $17.19$ & $\pm 0.01$ & $3.71$ & $\pm 0.02$ & $19.64$ & $\pm 0.35$ & $15.34$ & $\pm 0.00$ \\
\Algo{PPDSparse} & \multicolumn{2}{c}{$45.05$} & \multicolumn{2}{c}{$38.34$} & \multicolumn{2}{c|}{$34.90$} & \multicolumn{2}{c}{$0.00$} & \multicolumn{2}{c}{$0.00$} & \multicolumn{2}{c}{$0.00$} \\
\Algo{DiSMEC} & \multicolumn{2}{c}{$45.50$} & \multicolumn{2}{c}{$38.70$} & \multicolumn{2}{c|}{$35.50$} & \multicolumn{2}{c}{$0.00$} & \multicolumn{2}{c}{$0.00$} & \multicolumn{2}{c}{$0.00$} \\

\midrule
\Algo{Parabel-T=1} & $46.44$ & $\pm 0.07$ & $39.66$ & $\pm 0.06$ & $36.19$ & $\pm 0.05$ & $2.79$ & $\pm 0.03$ & $0.75$ & $\pm 0.01$ & $2.12$ & $\pm 0.00$ \\
\Algo{Parabel-T=3} & $46.62$ & $\pm 0.02$ & $39.78$ & $\pm 0.04$ & $36.37$ & $\pm 0.04$ & $9.01$ & $\pm 0.20$ & $2.61$ & $\pm 0.03$ & $6.36$ & $\pm 0.00$ \\
\Algo{XT-T=1} & $47.95$ & $\pm 0.03$ & $41.69$ & $\pm 0.02$ & $38.60$ & $\pm 0.01$ & $38.32$ & $\pm 1.84$ & $1.69$ & $\pm 0.05$ & $1.90$ & $\pm 0.00$ \\
\Algo{XT-T=3} & $48.28$ & $\pm 0.03$ & $41.93$ & $\pm 0.03$ & $38.87$ & $\pm 0.02$ & $112.03$ & $\pm 4.56$ & $4.56$ & $\pm 0.08$ & $2.70$ & $\pm 0.00$ \\
\Algo{PLT-T=1} & $49.55$ & $\pm 0.05$ & $43.08$ & $\pm 0.03$ & $39.90$ & $\pm 0.02$ & $2.58$ & $\pm 0.15$ & $9.89$ & $\pm 0.89$ & $0.95$ & $\pm 0.00$ \\
\Algo{PLT-T=3} & $49.65$ & $\pm 0.03$ & $43.18$ & $\pm 0.02$ & $39.97$ & $\pm 0.01$ & $7.90$ & $\pm 0.48$ & $31.10$ & $\pm 2.87$ & $2.86$ & $\pm 0.00$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}
\pagebreak

\specialrule{0.94pt}{0.4ex}{0.65ex}
\multicolumn{13}{c}{\textbf{\wikilshtc}} \\
\multicolumn{1}{c|}{} & \multicolumn{2}{c}{$p@1$ [\%]} & \multicolumn{2}{c}{$p@3$ [\%]} & \multicolumn{2}{c|}{$p@5$ [\%]} 
& \multicolumn{2}{c}{$T_{\textrm{train}}$ [h]} & \multicolumn{2}{c}{$T/N_{\textrm{test}}$ [ms]} & \multicolumn{2}{c}{$M_{\textrm{size}}$ [GB]} \\
\midrule
\Algo{FastXML} & $49.85$ & $\pm 0.00$ & $33.16$ & $\pm 0.01$ & $24.49$ & $\pm 0.01$ & $6.41$ & $\pm 0.13$ & $4.10$ & $\pm 0.04$ & $12.93$ & $\pm 0.00$ \\
\Algo{PfastreXML} & $58.50$ & $\pm 0.02$ & $37.69$ & $\pm 0.01$ & $27.57$ & $\pm 0.01$ & $6.25$ & $\pm 0.13$ & $4.00$ & $\pm 0.20$ & $14.20$ & $\pm 0.00$ \\
\Algo{PPDSparse} & \multicolumn{2}{c}{$64.13$} & \multicolumn{2}{c}{$42.10$} & \multicolumn{2}{c|}{$31.14$} & \multicolumn{2}{c}{$3.00$} & \multicolumn{2}{c}{$38.00$} & \multicolumn{2}{c}{$5.10$} \\
\Algo{DiSMEC} & \multicolumn{2}{c}{$64.94$} & \multicolumn{2}{c}{$42.71$} & \multicolumn{2}{c|}{$31.50$} & \multicolumn{2}{c}{$580.00$} & \multicolumn{2}{c}{$2600.00$} & \multicolumn{2}{c}{$3.80$} \\

\midrule
\Algo{Parabel-T=1} & $62.78$ & $\pm 0.02$ & $41.22$ & $\pm 0.02$ & $30.27$ & $\pm 0.01$ & $0.26$ & $\pm 0.01$ & $0.23$ & $\pm 0.00$ & $1.03$ & $\pm 0.00$ \\
\Algo{Parabel-T=3} & $64.95$ & $\pm 0.02$ & $43.21$ & $\pm 0.02$ & $32.01$ & $\pm 0.01$ & $0.81$ & $\pm 0.02$ & $1.27$ & $\pm 0.03$ & $3.10$ & $\pm 0.00$ \\
\Algo{XT-T=1} & $57.58$ & $\pm 0.06$ & $38.01$ & $\pm 0.04$ & $28.33$ & $\pm 0.02$ & $2.34$ & $\pm 0.17$ & $0.57$ & $\pm 0.01$ & $3.30$ & $\pm 0.00$ \\
\Algo{XT-T=3} & $60.20$ & $\pm 0.06$ & $40.12$ & $\pm 0.03$ & $29.97$ & $\pm 0.01$ & $6.51$ & $\pm 0.34$ & $2.32$ & $\pm 0.11$ & $4.50$ & $\pm 0.00$ \\
\Algo{PLT-T=1} & $61.96$ & $\pm 0.03$ & $40.77$ & $\pm 0.02$ & $30.19$ & $\pm 0.02$ & $2.95$ & $\pm 0.15$ & $1.77$ & $\pm 0.11$ & $2.73$ & $\pm 0.00$ \\
\Algo{PLT-T=3} & $63.73$ & $\pm 0.20$ & $42.12$ & $\pm 0.14$ & $31.21$ & $\pm 0.11$ & $8.06$ & $\pm 0.32$ & $5.07$ & $\pm 0.23$ & $8.18$ & $\pm 0.00$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}
\multicolumn{13}{c}{\textbf{\wikipedia}} \\
\multicolumn{1}{c|}{} & \multicolumn{2}{c}{$p@1$ [\%]} & \multicolumn{2}{c}{$p@3$ [\%]} & \multicolumn{2}{c|}{$p@5$ [\%]} 
& \multicolumn{2}{c}{$T_{\textrm{train}}$ [h]} & \multicolumn{2}{c}{$T/N_{\textrm{test}}$ [ms]} & \multicolumn{2}{c}{$M_{\textrm{size}}$ [GB]} \\
\midrule
\Algo{FastXML} & $49.32$ & $\pm 0.03$ & $33.48$ & $\pm 0.03$ & $25.84$ & $\pm 0.01$ & $51.48$ & $\pm 0.65$ & $15.35$ & $\pm 0.56$ & $59.69$ & $\pm 0.01$ \\
\Algo{PfastreXML} & $59.58$ & $\pm 0.02$ & $40.26$ & $\pm 0.01$ & $30.73$ & $\pm 0.01$ & $51.07$ & $\pm 0.92$ & $15.24$ & $\pm 0.24$ & $69.33$ & $\pm 0.01$ \\
\Algo{PPDSparse} & \multicolumn{2}{c}{$70.16$} & \multicolumn{2}{c}{$50.57$} & \multicolumn{2}{c|}{$39.66$} & \multicolumn{2}{c}{$26.00$} & \multicolumn{2}{c}{$130.00$} & \multicolumn{2}{c}{$4.00$} \\
\Algo{DiSMEC} & \multicolumn{2}{c}{$70.20$} & \multicolumn{2}{c}{$50.60$} & \multicolumn{2}{c|}{$39.70$} & \multicolumn{2}{c}{$6700.00$} & \multicolumn{2}{c}{$9800.00$} & \multicolumn{2}{c}{$14.80$} \\

\midrule
\Algo{Parabel-T=1} & $67.05$ & $\pm 0.14$ & $47.75$ & $\pm 0.10$ & $36.99$ & $\pm 0.08$ & $2.37$ & $\pm 0.05$ & $0.91$ & $\pm 0.03$ & $1.89$ & $\pm 0.00$ \\
\Algo{Parabel-T=3} & $68.66$ & $\pm 0.06$ & $49.48$ & $\pm 0.05$ & $38.60$ & $\pm 0.04$ & $7.33$ & $\pm 0.12$ & $3.44$ & $\pm 0.13$ & $5.69$ & $\pm 0.00$ \\
\Algo{XT-T=1} & $64.56$ & $\pm 0.06$ & $46.04$ & $\pm 0.06$ & $36.06$ & $\pm 0.04$ & $28.23$ & $\pm 1.41$ & $0.64$ & $\pm 0.01$ & $5.50$ & $\pm 0.00$ \\
\Algo{XT-T=3} & $67.45$ & $\pm 0.09$ & $48.54$ & $\pm 0.05$ & $38.11$ & $\pm 0.03$ & $56.54$ & $\pm 1.98$ & $1.87$ & $\pm 0.01$ & $7.50$ & $\pm 0.00$ \\
\Algo{PLT-T=1} & $66.20$ & $\pm 0.05$ & $47.14$ & $\pm 0.02$ & $36.83$ & $\pm 0.01$ & $16.10$ & $\pm 0.44$ & $6.67$ & $\pm 0.23$ & $8.89$ & $\pm 0.00$ \\
\Algo{PLT-T=3} & $67.86$ & $\pm 0.03$ & $48.55$ & $\pm 0.03$ & $37.95$ & $\pm 0.02$ & $48.06$ & $\pm 0.24$ & $22.72$ & $\pm 0.10$ & $26.71$ & $\pm 0.00$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}
\multicolumn{13}{c}{\textbf{\amazon}} \\
\multicolumn{1}{c|}{} & \multicolumn{2}{c}{$p@1$ [\%]} & \multicolumn{2}{c}{$p@3$ [\%]} & \multicolumn{2}{c|}{$p@5$ [\%]} 
& \multicolumn{2}{c}{$T_{\textrm{train}}$ [h]} & \multicolumn{2}{c}{$T/N_{\textrm{test}}$ [ms]} & \multicolumn{2}{c}{$M_{\textrm{size}}$ [GB]} \\
\midrule
\Algo{FastXML} & $36.90$ & $\pm 0.02$ & $33.22$ & $\pm 0.01$ & $30.44$ & $\pm 0.01$ & $2.80$ & $\pm 0.03$ & $8.57$ & $\pm 0.20$ & $9.54$ & $\pm 0.00$ \\
\Algo{PfastreXML} & $36.97$ & $\pm 0.02$ & $34.18$ & $\pm 0.01$ & $32.05$ & $\pm 0.01$ & $3.01$ & $\pm 0.03$ & $9.96$ & $\pm 0.14$ & $10.98$ & $\pm 0.00$ \\
\Algo{PPDSparse} & \multicolumn{2}{c}{$45.32$} & \multicolumn{2}{c}{$40.37$} & \multicolumn{2}{c|}{$36.92$} & \multicolumn{2}{c}{$2.00$} & \multicolumn{2}{c}{$90.00$} & \multicolumn{2}{c}{$6.00$} \\
\Algo{DiSMEC} & \multicolumn{2}{c}{$45.37$} & \multicolumn{2}{c}{$40.40$} & \multicolumn{2}{c|}{$36.96$} & \multicolumn{2}{c}{$350.00$} & \multicolumn{2}{c}{$1900.00$} & \multicolumn{2}{c}{$3.80$} \\

\midrule
\Algo{Parabel-T=1} & $43.13$ & $\pm 0.02$ & $37.94$ & $\pm 0.03$ & $34.00$ & $\pm 0.00$ & $0.13$ & $\pm 0.00$ & $0.30$ & $\pm 0.01$ & $0.65$ & $\pm 0.00$ \\
\Algo{Parabel-T=3} & $44.70$ & $\pm 0.04$ & $39.66$ & $\pm 0.04$ & $35.85$ & $\pm 0.04$ & $0.39$ & $\pm 0.00$ & $1.57$ & $\pm 0.05$ & $1.95$ & $\pm 0.00$ \\
\Algo{XT-T=1} & $40.24$ & $\pm 0.03$ & $35.84$ & $\pm 0.04$ & $32.61$ & $\pm 0.05$ & $6.27$ & $\pm 0.49$ & $1.18$ & $\pm 0.01$ & $1.60$ & $\pm 0.00$ \\
\Algo{XT-T=3} & $42.64$ & $\pm 0.02$ & $38.14$ & $\pm 0.03$ & $34.75$ & $\pm 0.01$ & $16.88$ & $\pm 0.72$ & $5.14$ & $\pm 0.16$ & $4.20$ & $\pm 0.00$ \\
\Algo{PLT-T=1} & $43.54$ & $\pm 0.01$ & $38.71$ & $\pm 0.02$ & $35.15$ & $\pm 0.03$ & $0.56$ & $\pm 0.00$ & $4.13$ & $\pm 0.28$ & $2.26$ & $\pm 0.00$ \\
\Algo{PLT-T=3} & $44.55$ & $\pm 0.12$ & $39.74$ & $\pm 0.10$ & $36.17$ & $\pm 0.10$ & $1.72$ & $\pm 0.04$ & $12.63$ & $\pm 0.48$ & $6.78$ & $\pm 0.00$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}
\multicolumn{13}{c}{\textbf{\amazonlarge}} \\
\multicolumn{1}{c|}{} & \multicolumn{2}{c}{$p@1$ [\%]} & \multicolumn{2}{c}{$p@3$ [\%]} & \multicolumn{2}{c|}{$p@5$ [\%]} 
& \multicolumn{2}{c}{$T_{\textrm{train}}$ [h]} & \multicolumn{2}{c}{$T/N_{\textrm{test}}$ [ms]} & \multicolumn{2}{c}{$M_{\textrm{size}}$ [GB]} \\
\midrule
\Algo{FastXML} & $45.26$ & $\pm 0.01$ & $41.96$ & $\pm 0.00$ & $39.80$ & $\pm 0.01$ & $18.19$ & $\pm 1.01$ & $68.77$ & $\pm 4.16$ & $30.70$ & $\pm 0.00$ \\
\Algo{PfastreXML} & $32.62$ & $\pm 0.01$ & $32.67$ & $\pm 0.01$ & $32.35$ & $\pm 0.01$ & $19.07$ & $\pm 0.92$ & $78.83$ & $\pm 3.93$ & $41.88$ & $\pm 0.00$ \\
%\Algo{PPDSparse} & \multicolumn{2}{c}{$0.00$} & \multicolumn{2}{c}{$0.00$} & \multicolumn{2}{c|}{$0.00$} & \multicolumn{2}{c}{$0.00$} & \multicolumn{2}{c}{$0.00$} & \multicolumn{2}{c}{$0.00$} \\
\Algo{DiSMEC} & \multicolumn{2}{c}{$47.77$} & \multicolumn{2}{c}{$44.96$} & \multicolumn{2}{c|}{$42.80$} & \multicolumn{2}{c}{$4700.00$} & \multicolumn{2}{c}{$16430.00$} & \multicolumn{2}{c}{$39.70$} \\

\midrule
\Algo{Parabel-T=1} & $46.14$ & $\pm 0.01$ & $43.32$ & $\pm 0.01$ & $41.20$ & $\pm 0.01$ & $1.61$ & $\pm 0.02$ & $0.27$ & $\pm 0.01$ & $10.48$ & $\pm 0.00$ \\
\Algo{Parabel-T=3} & $47.52$ & $\pm 0.01$ & $44.69$ & $\pm 0.01$ & $42.57$ & $\pm 0.00$ & $5.20$ & $\pm 0.01$ & $1.53$ & $\pm 0.02$ & $31.43$ & $\pm 0.00$ \\
\Algo{XT-T=1} & $39.29$ & $\pm 0.03$ & $36.53$ & $\pm 0.02$ & $34.65$ & $\pm 0.01$ & $36.07$ & $\pm 2.05$ & $0.91$ & $\pm 0.01$ & $6.20$ & $\pm 0.00$ \\
\Algo{XT-T=3} & $41.14$ & $\pm 0.02$ & $38.36$ & $\pm 0.03$ & $36.43$ & $\pm 0.03$ & $100.33$ & $\pm 1.88$ & $3.05$ & $\pm 0.06$ & $17.00$ & $\pm 0.00$ \\
\Algo{PLT-T=1} & $46.09$ & $\pm 0.02$ & $43.11$ & $\pm 0.01$ & $40.98$ & $\pm 0.01$ & $7.07$ & $\pm 0.56$ & $3.26$ & $\pm 0.08$ & $20.84$ & $\pm 0.00$ \\
\Algo{PLT-T=3} & $47.02$ & $\pm 0.01$ & $44.00$ & $\pm 0.02$ & $41.82$ & $\pm 0.02$ & $21.55$ & $\pm 0.28$ & $13.58$ & $\pm 0.14$ & $62.53$ & $\pm 0.00$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}
\caption{Results of PLT and compared methods.}
\label{tab:plt-vs-sota}
\end{longtable}
\end{center}


==> tables/table-trees-arity-logistic.tex <==

\begin{table}[H]
\footnotesize{
\resizebox{\textwidth}{!}{
\tabcolsep=5pt
\begin{tabular}{l|r@{}lr@{}lr@{}l|r@{}lr@{}lr@{}l}

\specialrule{0.94pt}{0.4ex}{0.65ex}
Arity & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{16} & \multicolumn{2}{c|}{64} 
& \multicolumn{2}{c}{2} & \multicolumn{2}{c}{16} & \multicolumn{2}{c}{64} \\
\specialrule{0.94pt}{0.4ex}{0.65ex}
& \multicolumn{6}{c|}{$p@1$ [\%]}
& \multicolumn{6}{c}{$T/N_{\textrm{test}}$ [ms]} \\
\midrule
% \eurlex & $80.51$ & $\pm 0.16$ & $81.06$ & $\pm 0.03$ & \boldmath$81.20$ & \boldmath$\pm 0.13$ & $0.39$ & $\pm 0.03$ & \boldmath$0.23$ & \boldmath$\pm 0.02$ & $0.28$ & $\pm 0.03$ \\
% \amazoncatsmall & $93.04$ & $\pm 0.02$ & $93.15$ & $\pm 0.04$ & \boldmath$93.19$ & \boldmath$\pm 0.01$ & \boldmath$0.32$ & \boldmath$\pm 0.03$ & $0.34$ & $\pm 0.03$ & $0.43$ & $\pm 0.04$ \\
% \wikiten & $85.36$ & $\pm 0.09$ & $85.85$ & $\pm 0.06$ & \boldmath$86.03$ & \boldmath$\pm 0.07$ & \boldmath$5.35$ & \boldmath$\pm 0.32$ & $5.63$ & $\pm 0.33$ & $7.34$ & $\pm 0.62$ \\
% \deliciouslarge & $49.55$ & $\pm 0.05$ & \boldmath$49.56$ & \boldmath$\pm 0.04$ & $49.51$ & $\pm 0.04$ & \boldmath$9.89$ & \boldmath$\pm 0.89$ & $12.74$ & $\pm 1.69$ & $11.77$ & $\pm 0.61$ \\
\wikilshtc & $61.96$ & $\pm 0.03$ & $63.16$ & $\pm 0.03$ & \boldmath$63.62$ & \boldmath$\pm 0.03$ & $1.77$ & $\pm 0.11$ & \boldmath$1.26$ & \boldmath$\pm 0.03$ & $1.91$ & $\pm 0.19$ \\
\wikipedia & $66.20$ & $\pm 0.05$ & $67.36$ & $\pm 0.10$ & \boldmath$67.49$ & \boldmath$\pm 0.05$ & $6.67$ & $\pm 0.23$ & \boldmath$6.47$ & \boldmath$\pm 0.30$ & $9.02$ & $\pm 0.39$ \\
\amazon & \boldmath$43.54$ & \boldmath$\pm 0.01$ & $43.33$ & $\pm 0.04$ & $43.53$ & $\pm 0.05$ & $4.13$ & $\pm 0.28$ & \boldmath$2.91$ & \boldmath$\pm 0.17$ & $5.12$ & $\pm 0.24$ \\
\amazonlarge & $46.09$ & $\pm 0.02$ & $46.74$ & $\pm 0.01$ & \boldmath$46.97$ & \boldmath$\pm 0.01$ & $3.26$ & $\pm 0.08$ & \boldmath$3.06$ & \boldmath$\pm 0.04$ & $4.19$ & $\pm 0.16$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}
& \multicolumn{6}{c|}{$T_{\textrm{train}}$ [h]}
& \multicolumn{6}{c}{$M_{\textrm{size}}$ [GB]} \\
\midrule
% \eurlex & \boldmath$0.02$ & \boldmath$\pm 0.00$ & $0.02$ & $\pm 0.00$ & $0.02$ & $\pm 0.00$ & \boldmath$0.02$ & \boldmath$\pm 0.00$ & $0.02$ & $\pm 0.00$ & $0.02$ & $\pm 0.00$ \\
% \amazoncatsmall & \boldmath$0.72$ & \boldmath$\pm 0.02$ & $0.82$ & $\pm 0.05$ & $1.09$ & $\pm 0.03$ & $0.35$ & $\pm 0.00$ & \boldmath$0.34$ & \boldmath$\pm 0.00$ & $0.34$ & $\pm 0.00$ \\
% \wikiten & $0.21$ & $\pm 0.00$ & \boldmath$0.20$ & \boldmath$\pm 0.01$ & $0.43$ & $\pm 0.04$ & $0.58$ & $\pm 0.00$ & \boldmath$0.50$ & \boldmath$\pm 0.00$ & $0.51$ & $\pm 0.00$ \\
% \deliciouslarge & \boldmath$2.58$ & \boldmath$\pm 0.15$ & $5.49$ & $\pm 0.36$ & $9.21$ & $\pm 0.90$ & $0.95$ & $\pm 0.00$ & $0.93$ & $\pm 0.00$ & \boldmath$0.91$ & \boldmath$\pm 0.00$ \\
\wikilshtc & \boldmath$2.95$ & \boldmath$\pm 0.15$ & $3.71$ & $\pm 0.13$ & $7.13$ & $\pm 0.41$ & $2.73$ & $\pm 0.00$ & $2.65$ & $\pm 0.00$ & \boldmath$2.62$ & \boldmath$\pm 0.00$ \\
\wikipedia & \boldmath$16.10$ & \boldmath$\pm 0.44$ & $26.28$ & $\pm 0.40$ & $46.84$ & $\pm 2.94$ & $8.89$ & $\pm 0.00$ & $8.20$ & $\pm 0.00$ & \boldmath$8.13$ & \boldmath$\pm 0.00$ \\
\amazon & \boldmath$0.56$ & \boldmath$\pm 0.00$ & $0.78$ & $\pm 0.03$ & $2.17$ & $\pm 0.12$ & $2.26$ & $\pm 0.00$ & $1.68$ & $\pm 0.00$ & \boldmath$1.60$ & \boldmath$\pm 0.00$ \\
\amazonlarge & \boldmath$7.07$ & \boldmath$\pm 0.56$ & $9.80$ & $\pm 0.10$ & $23.69$ & $\pm 1.09$ & $20.84$ & $\pm 0.00$ & $20.32$ & $\pm 0.00$ & \boldmath$20.17$ & \boldmath$\pm 0.00$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}
\end{tabular}}}
\caption{\Precatk{1}, average prediction time per example, training time and model size for $k$-means trees with $k = 2,16,64$ for logistic loss.}
\label{tab:k-means-tree-arity-logistic}
\end{table}


==> tables/table-trees-arity-sh.tex <==

\begin{table}[H]
\centering

\footnotesize{
\resizebox{\textwidth}{!}{
\tabcolsep=5pt
\begin{tabular}{l|r@{}lr@{}lr@{}l|r@{}lr@{}lr@{}l}
\specialrule{0.94pt}{0.4ex}{0.65ex}
Arity & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{16} & \multicolumn{2}{c|}{64}
& \multicolumn{2}{c}{2} & \multicolumn{2}{c}{16} & \multicolumn{2}{c}{64} \\
\specialrule{0.94pt}{0.4ex}{0.65ex}
& \multicolumn{6}{c|}{$p@1$ [\%]}
& \multicolumn{6}{c}{$T/N_{\textrm{test}}$ [ms]} \\
\midrule
%\eurlex & $80.17$ & $\pm 0.27$ & $81.62$ & $\pm 0.15$ & \boldmath$81.68$ & \boldmath$\pm 0.24$ & $0.24$ & $\pm 0.02$ & \boldmath$0.18$ & \boldmath$\pm 0.01$ & $0.27$ & $\pm 0.02$ \\
%\amazoncatsmall & $92.40$ & $\pm 0.04$ & $92.39$ & $\pm 0.06$ & \boldmath$92.46$ & \boldmath$\pm 0.07$ & \boldmath$0.19$ & \boldmath$\pm 0.00$ & $0.23$ & $\pm 0.01$ & $0.31$ & $\pm 0.03$ \\
%\wikiten & $84.17$ & $\pm 0.10$ & $84.30$ & $\pm 0.07$ & \boldmath$84.62$ & \boldmath$\pm 0.07$ & \boldmath$2.87$ & \boldmath$\pm 0.08$ & $2.95$ & $\pm 0.20$ & $4.14$ & $\pm 0.28$ \\
%\deliciouslarge & $46.30$ & $\pm 0.07$ & $46.19$ & $\pm 0.08$ & \boldmath$46.31$ & \boldmath$\pm 0.06$ & \boldmath$10.07$ & \boldmath$\pm 0.23$ & $12.59$ & $\pm 0.51$ & $11.83$ & $\pm 0.48$ \\
\wikilshtc & $62.78$ & $\pm 0.03$ & $64.17$ & $\pm 0.05$ & \boldmath$64.61$ & \boldmath$\pm 0.04$ & \boldmath$0.86$ & \boldmath$\pm 0.06$ & $0.90$ & $\pm 0.07$ & $1.42$ & $\pm 0.05$ \\
\wikipedia & $66.77$ & $\pm 0.08$ & \boldmath$68.16$ & \boldmath$\pm 0.10$ & $68.02$ & $\pm 0.01$ & \boldmath$2.86$ & \boldmath$\pm 0.07$ & $4.41$ & $\pm 0.12$ & $5.55$ & $\pm 0.00$ \\
\amazon & $43.31$ & $\pm 0.03$ & $43.88$ & $\pm 0.05$ & \boldmath$44.03$ & \boldmath$\pm 0.05$ & \boldmath$1.32$ & \boldmath$\pm 0.08$ & $1.73$ & $\pm 0.15$ & $2.68$ & $\pm 0.17$ \\
\amazonlarge & $46.23$ & $\pm 0.01$ & $46.98$ & $\pm 0.01$ & \boldmath$47.33$ & \boldmath$\pm 0.00$ & \boldmath$1.96$ & \boldmath$\pm 0.05$ & $2.39$ & $\pm 0.09$ & $2.56$ & $\pm 0.00$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}

& \multicolumn{6}{c|}{$T_{\textrm{train}}$ [h]}
& \multicolumn{6}{c}{$M_{\textrm{size}}$ [GB]} \\
\midrule
%\eurlex & \boldmath$0.01$ & \boldmath$\pm 0.00$ & $0.01$ & $\pm 0.00$ & $0.01$ & $\pm 0.00$ & \boldmath$0.00$ & \boldmath$\pm 0.00$ & $0.00$ & $\pm 0.00$ & $0.01$ & $\pm 0.00$ \\
%\amazoncatsmall & \boldmath$0.29$ & \boldmath$\pm 0.00$ & $0.38$ & $\pm 0.04$ & $0.47$ & $\pm 0.03$ & $0.19$ & $\pm 0.00$ & \boldmath$0.18$ & \boldmath$\pm 0.00$ & $0.18$ & $\pm 0.00$ \\
%\wikiten & \boldmath$0.11$ & \boldmath$\pm 0.00$ & $0.16$ & $\pm 0.00$ & $0.36$ & $\pm 0.02$ & $0.06$ & $\pm 0.00$ & $0.05$ & $\pm 0.00$ & \boldmath$0.04$ & \boldmath$\pm 0.00$ \\
%\deliciouslarge & \boldmath$5.51$ & \boldmath$\pm 0.29$ & $9.07$ & $\pm 0.76$ & $12.23$ & $\pm 0.78$ & $1.82$ & $\pm 0.00$ & $1.77$ & $\pm 0.00$ & \boldmath$1.74$ & \boldmath$\pm 0.00$ \\
\wikilshtc & \boldmath$1.60$ & \boldmath$\pm 0.06$ & $2.18$ & $\pm 0.07$ & $3.85$ & $\pm 0.17$ & $0.97$ & $\pm 0.00$ & $0.90$ & $\pm 0.00$ & \boldmath$0.88$ & \boldmath$\pm 0.00$ \\
\wikipedia & \boldmath$9.48$ & \boldmath$\pm 0.33$ & $15.91$ & $\pm 0.55$ & $28.68$ & $\pm 0.74$ & $1.78$ & $\pm 0.00$ & $1.52$ & $\pm 0.00$ & \boldmath$1.49$ & \boldmath$\pm 0.00$ \\
\amazon & \boldmath$0.40$ & \boldmath$\pm 0.01$ & $0.64$ & $\pm 0.02$ & $1.57$ & $\pm 0.04$ & $0.63$ & $\pm 0.00$ & $0.55$ & $\pm 0.00$ & \boldmath$0.52$ & \boldmath$\pm 0.00$ \\
\amazonlarge & \boldmath$5.44$ & \boldmath$\pm 0.13$ & $9.82$ & $\pm 0.23$ & $20.82$ & $\pm 0.00$ & $9.86$ & $\pm 0.00$ & $9.36$ & $\pm 0.00$ & \boldmath$9.24$ & \boldmath$\pm 0.00$ \\
\specialrule{0.94pt}{0.4ex}{0.65ex}
\end{tabular}}}

\caption{Precision$@1$, average prediction time per example, training time and model size for $k$-means trees with $k = 2,16,64$ and squared hinge loss.}
\label{tab:k-means-tree-arity}
\end{table}


==> tables/table-trees-arity.tex <==

\begin{table}[H]
\centering

\begin{subtable}{\textwidth}
\footnotesize{
\resizebox{\textwidth}{!}{
\tabcolsep=5pt
\begin{tabular}{l|r@{}lr@{}lr@{}l|r@{}lr@{}lr@{}l}

\specialrule{0.94pt}{0.4ex}{0.65ex}
Arity & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{16} & \multicolumn{2}{c|}{64} 
& \multicolumn{2}{c}{2} & \multicolumn{2}{c}{16} & \multicolumn{2}{c}{64} \\
\specialrule{0.94pt}{0.4ex}{0.65ex}
& \multicolumn{6}{c|}{$p@1$ [\%]}
& \multicolumn{6}{c}{$T/N_{\textrm{test}}$ [ms]} \\
\midrule
% \eurlex & $80.51$ & $\pm 0.16$ & $81.06$ & $\pm 0.03$ & \boldmath$81.20$ & \boldmath$\pm 0.13$ & $0.39$ & $\pm 0.03$ & \boldmath$0.23$ & \boldmath$\pm 0.02$ & $0.28$ & $\pm 0.03$ \\
% \amazoncatsmall & $93.04$ & $\pm 0.02$ & $93.15$ & $\pm 0.04$ & \boldmath$93.19$ & \boldmath$\pm 0.01$ & \boldmath$0.32$ & \boldmath$\pm 0.03$ & $0.34$ & $\pm 0.03$ & $0.43$ & $\pm 0.04$ \\
% \wikiten & $85.36$ & $\pm 0.09$ & $85.85$ & $\pm 0.06$ & \boldmath$86.03$ & \boldmath$\pm 0.07$ & \boldmath$5.35$ & \boldmath$\pm 0.32$ & $5.63$ & $\pm 0.33$ & $7.34$ & $\pm 0.62$ \\
% \deliciouslarge & $49.55$ & $\pm 0.05$ & \boldmath$49.56$ & \boldmath$\pm 0.04$ & $49.51$ & $\pm 0.04$ & \boldmath$9.89$ & \boldmath$\pm 0.89$ & $12.74$ & $\pm 1.69$ & $11.77$ & $\pm 0.61$ \\
\wikilshtc & $61.96$ & $\pm 0.03$ & $63.16$ & $\pm 0.03$ & \boldmath$63.62$ & \boldmath$\pm 0.03$ & $1.77$ & $\pm 0.11$ & \boldmath$1.26$ & \boldmath$\pm 0.03$ & $1.91$ & $\pm 0.19$ \\
\wikipedia & $66.20$ & $\pm 0.05$ & $67.36$ & $\pm 0.10$ & \boldmath$67.49$ & \boldmath$\pm 0.05$ & $6.67$ & $\pm 0.23$ & \boldmath$6.47$ & \boldmath$\pm 0.30$ & $9.02$ & $\pm 0.39$ \\
\amazon & \boldmath$43.54$ & \boldmath$\pm 0.01$ & $43.33$ & $\pm 0.04$ & $43.53$ & $\pm 0.05$ & $4.13$ & $\pm 0.28$ & \boldmath$2.91$ & \boldmath$\pm 0.17$ & $5.12$ & $\pm 0.24$ \\
\amazonlarge & $46.09$ & $\pm 0.02$ & $46.74$ & $\pm 0.01$ & \boldmath$46.97$ & \boldmath$\pm 0.01$ & $3.26$ & $\pm 0.08$ & \boldmath$3.06$ & \boldmath$\pm 0.04$ & $4.19$ & $\pm 0.16$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}
& \multicolumn{6}{c|}{$T_{\textrm{train}}$ [h]}
& \multicolumn{6}{c}{$M_{\textrm{size}}$ [GB]} \\
\midrule
% \eurlex & \boldmath$0.02$ & \boldmath$\pm 0.00$ & $0.02$ & $\pm 0.00$ & $0.02$ & $\pm 0.00$ & \boldmath$0.02$ & \boldmath$\pm 0.00$ & $0.02$ & $\pm 0.00$ & $0.02$ & $\pm 0.00$ \\
% \amazoncatsmall & \boldmath$0.72$ & \boldmath$\pm 0.02$ & $0.82$ & $\pm 0.05$ & $1.09$ & $\pm 0.03$ & $0.35$ & $\pm 0.00$ & \boldmath$0.34$ & \boldmath$\pm 0.00$ & $0.34$ & $\pm 0.00$ \\
% \wikiten & $0.21$ & $\pm 0.00$ & \boldmath$0.20$ & \boldmath$\pm 0.01$ & $0.43$ & $\pm 0.04$ & $0.58$ & $\pm 0.00$ & \boldmath$0.50$ & \boldmath$\pm 0.00$ & $0.51$ & $\pm 0.00$ \\
% \deliciouslarge & \boldmath$2.58$ & \boldmath$\pm 0.15$ & $5.49$ & $\pm 0.36$ & $9.21$ & $\pm 0.90$ & $0.95$ & $\pm 0.00$ & $0.93$ & $\pm 0.00$ & \boldmath$0.91$ & \boldmath$\pm 0.00$ \\
\wikilshtc & \boldmath$2.95$ & \boldmath$\pm 0.15$ & $3.71$ & $\pm 0.13$ & $7.13$ & $\pm 0.41$ & $2.73$ & $\pm 0.00$ & $2.65$ & $\pm 0.00$ & \boldmath$2.62$ & \boldmath$\pm 0.00$ \\
\wikipedia & \boldmath$16.10$ & \boldmath$\pm 0.44$ & $26.28$ & $\pm 0.40$ & $46.84$ & $\pm 2.94$ & $8.89$ & $\pm 0.00$ & $8.20$ & $\pm 0.00$ & \boldmath$8.13$ & \boldmath$\pm 0.00$ \\
\amazon & \boldmath$0.56$ & \boldmath$\pm 0.00$ & $0.78$ & $\pm 0.03$ & $2.17$ & $\pm 0.12$ & $2.26$ & $\pm 0.00$ & $1.68$ & $\pm 0.00$ & \boldmath$1.60$ & \boldmath$\pm 0.00$ \\
\amazonlarge & \boldmath$7.07$ & \boldmath$\pm 0.56$ & $9.80$ & $\pm 0.10$ & $23.69$ & $\pm 1.09$ & $20.84$ & $\pm 0.00$ & $20.32$ & $\pm 0.00$ & \boldmath$20.17$ & \boldmath$\pm 0.00$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}
\end{tabular}}}

\caption{Results for logistic loss.}
\end{subtable}

\vspace{12pt}

\begin{subtable}{\textwidth}
\footnotesize{
\resizebox{\textwidth}{!}{
\tabcolsep=5pt
\begin{tabular}{l|r@{}lr@{}lr@{}l|r@{}lr@{}lr@{}l}
\specialrule{0.94pt}{0.4ex}{0.65ex}
Arity & \multicolumn{2}{c}{2} & \multicolumn{2}{c}{16} & \multicolumn{2}{c|}{64}
& \multicolumn{2}{c}{2} & \multicolumn{2}{c}{16} & \multicolumn{2}{c}{64} \\
\specialrule{0.94pt}{0.4ex}{0.65ex}
& \multicolumn{6}{c|}{$p@1$ [\%]}
& \multicolumn{6}{c}{$T/N_{\textrm{test}}$ [ms]} \\
\midrule
%\eurlex & $80.17$ & $\pm 0.27$ & $81.62$ & $\pm 0.15$ & \boldmath$81.68$ & \boldmath$\pm 0.24$ & $0.24$ & $\pm 0.02$ & \boldmath$0.18$ & \boldmath$\pm 0.01$ & $0.27$ & $\pm 0.02$ \\
%\amazoncatsmall & $92.40$ & $\pm 0.04$ & $92.39$ & $\pm 0.06$ & \boldmath$92.46$ & \boldmath$\pm 0.07$ & \boldmath$0.19$ & \boldmath$\pm 0.00$ & $0.23$ & $\pm 0.01$ & $0.31$ & $\pm 0.03$ \\
%\wikiten & $84.17$ & $\pm 0.10$ & $84.30$ & $\pm 0.07$ & \boldmath$84.62$ & \boldmath$\pm 0.07$ & \boldmath$2.87$ & \boldmath$\pm 0.08$ & $2.95$ & $\pm 0.20$ & $4.14$ & $\pm 0.28$ \\
%\deliciouslarge & $46.30$ & $\pm 0.07$ & $46.19$ & $\pm 0.08$ & \boldmath$46.31$ & \boldmath$\pm 0.06$ & \boldmath$10.07$ & \boldmath$\pm 0.23$ & $12.59$ & $\pm 0.51$ & $11.83$ & $\pm 0.48$ \\
\wikilshtc & $62.78$ & $\pm 0.03$ & $64.17$ & $\pm 0.05$ & \boldmath$64.61$ & \boldmath$\pm 0.04$ & \boldmath$0.86$ & \boldmath$\pm 0.06$ & $0.90$ & $\pm 0.07$ & $1.42$ & $\pm 0.05$ \\
\wikipedia & $66.77$ & $\pm 0.08$ & \boldmath$68.16$ & \boldmath$\pm 0.10$ & $68.02$ & $\pm 0.01$ & \boldmath$2.86$ & \boldmath$\pm 0.07$ & $4.41$ & $\pm 0.12$ & $5.55$ & $\pm 0.00$ \\
\amazon & $43.31$ & $\pm 0.03$ & $43.88$ & $\pm 0.05$ & \boldmath$44.03$ & \boldmath$\pm 0.05$ & \boldmath$1.32$ & \boldmath$\pm 0.08$ & $1.73$ & $\pm 0.15$ & $2.68$ & $\pm 0.17$ \\
\amazonlarge & $46.23$ & $\pm 0.01$ & $46.98$ & $\pm 0.01$ & \boldmath$47.33$ & \boldmath$\pm 0.00$ & \boldmath$1.96$ & \boldmath$\pm 0.05$ & $2.39$ & $\pm 0.09$ & $2.56$ & $\pm 0.00$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}

& \multicolumn{6}{c|}{$T_{\textrm{train}}$ [h]}
& \multicolumn{6}{c}{$M_{\textrm{size}}$ [GB]} \\
\midrule
%\eurlex & \boldmath$0.01$ & \boldmath$\pm 0.00$ & $0.01$ & $\pm 0.00$ & $0.01$ & $\pm 0.00$ & \boldmath$0.00$ & \boldmath$\pm 0.00$ & $0.00$ & $\pm 0.00$ & $0.01$ & $\pm 0.00$ \\
%\amazoncatsmall & \boldmath$0.29$ & \boldmath$\pm 0.00$ & $0.38$ & $\pm 0.04$ & $0.47$ & $\pm 0.03$ & $0.19$ & $\pm 0.00$ & \boldmath$0.18$ & \boldmath$\pm 0.00$ & $0.18$ & $\pm 0.00$ \\
%\wikiten & \boldmath$0.11$ & \boldmath$\pm 0.00$ & $0.16$ & $\pm 0.00$ & $0.36$ & $\pm 0.02$ & $0.06$ & $\pm 0.00$ & $0.05$ & $\pm 0.00$ & \boldmath$0.04$ & \boldmath$\pm 0.00$ \\
%\deliciouslarge & \boldmath$5.51$ & \boldmath$\pm 0.29$ & $9.07$ & $\pm 0.76$ & $12.23$ & $\pm 0.78$ & $1.82$ & $\pm 0.00$ & $1.77$ & $\pm 0.00$ & \boldmath$1.74$ & \boldmath$\pm 0.00$ \\
\wikilshtc & \boldmath$1.60$ & \boldmath$\pm 0.06$ & $2.18$ & $\pm 0.07$ & $3.85$ & $\pm 0.17$ & $0.97$ & $\pm 0.00$ & $0.90$ & $\pm 0.00$ & \boldmath$0.88$ & \boldmath$\pm 0.00$ \\
\wikipedia & \boldmath$9.48$ & \boldmath$\pm 0.33$ & $15.91$ & $\pm 0.55$ & $28.68$ & $\pm 0.74$ & $1.78$ & $\pm 0.00$ & $1.52$ & $\pm 0.00$ & \boldmath$1.49$ & \boldmath$\pm 0.00$ \\
\amazon & \boldmath$0.40$ & \boldmath$\pm 0.01$ & $0.64$ & $\pm 0.02$ & $1.57$ & $\pm 0.04$ & $0.63$ & $\pm 0.00$ & $0.55$ & $\pm 0.00$ & \boldmath$0.52$ & \boldmath$\pm 0.00$ \\
\amazonlarge & \boldmath$5.44$ & \boldmath$\pm 0.13$ & $9.82$ & $\pm 0.23$ & $20.82$ & $\pm 0.00$ & $9.86$ & $\pm 0.00$ & $9.36$ & $\pm 0.00$ & \boldmath$9.24$ & \boldmath$\pm 0.00$ \\
\specialrule{0.94pt}{0.4ex}{0.65ex}
\end{tabular}}}
\caption{Results for squared hinge loss.}
\end{subtable}

\caption{Precision$@1$, average prediction time per example, training time and model size for $k$-means trees with $k = 2,16,64$.}
\label{tab:k-means-tree-arity}
\end{table}


==> tables/table-trees-comp.tex <==
\begin{table}[h]
\centering
\footnotesize{
\resizebox{\textwidth}{!}{
\tabcolsep=5pt
\begin{tabular}{l|r@{}lr@{}l|r@{}lr@{}l|r@{}lr@{}l}
\toprule
& \multicolumn{4}{c|}{$T_{\textrm{train}}$ [h]}
& \multicolumn{4}{c|}{$T/N_{\textrm{test}}$ [ms]}
& \multicolumn{4}{c}{$M_{\textrm{size}}$ [GB]} \\
& \multicolumn{2}{c}{random} & \multicolumn{2}{c|}{k-means}
& \multicolumn{2}{c}{random} & \multicolumn{2}{c|}{k-means}
& \multicolumn{2}{c}{random} & \multicolumn{2}{c}{k-means} \\
\midrule
\eurlex & \boldmath$0.02$ & \boldmath$\pm 0.00$ & $0.02$ & $\pm 0.00$ & \boldmath$0.27$ & \boldmath$\pm 0.02$ & $0.39$ & $\pm 0.03$ & \boldmath$0.02$ & \boldmath$\pm 0.00$ & $0.02$ & $\pm 0.00$ \\
\amazoncatsmall & $0.84$ & $\pm 0.03$ & \boldmath$0.72$ & \boldmath$\pm 0.02$ & $0.37$ & $\pm 0.02$ & \boldmath$0.32$ & \boldmath$\pm 0.03$ & $0.40$ & $\pm 0.00$ & \boldmath$0.35$ & \boldmath$\pm 0.00$ \\
\wikiten & \boldmath$0.19$ & \boldmath$\pm 0.01$ & $0.21$ & $\pm 0.00$ & \boldmath$2.59$ & \boldmath$\pm 0.21$ & $5.35$ & $\pm 0.32$ & $0.62$ & $\pm 0.00$ & \boldmath$0.58$ & \boldmath$\pm 0.00$ \\
\deliciouslarge & $5.26$ & $\pm 0.26$ & \boldmath$2.58$ & \boldmath$\pm 0.15$ & \boldmath$5.24$ & \boldmath$\pm 0.43$ & $9.89$ & $\pm 0.89$ & $1.30$ & $\pm 0.00$ & \boldmath$0.95$ & \boldmath$\pm 0.00$ \\
\wikilshtc & $3.01$ & $\pm 0.16$ & \boldmath$2.95$ & \boldmath$\pm 0.15$ & \boldmath$1.36$ & \boldmath$\pm 0.13$ & $1.77$ & $\pm 0.11$ & $3.25$ & $\pm 0.00$ & \boldmath$2.73$ & \boldmath$\pm 0.00$ \\
\wikipedia & $22.07$ & $\pm 0.59$ & \boldmath$16.10$ & \boldmath$\pm 0.44$ & $10.65$ & $\pm 0.52$ & \boldmath$6.67$ & \boldmath$\pm 0.23$ & $12.00$ & $\pm 0.00$ & \boldmath$8.89$ & \boldmath$\pm 0.00$ \\
\amazon & $1.02$ & $\pm 0.02$ & \boldmath$0.56$ & \boldmath$\pm 0.00$ & $4.74$ & $\pm 0.22$ & \boldmath$4.13$ & \boldmath$\pm 0.28$ & $3.00$ & $\pm 0.00$ & \boldmath$2.26$ & \boldmath$\pm 0.00$ \\
\amazonlarge & $48.09$ & $\pm 1.72$ & \boldmath$7.07$ & \boldmath$\pm 0.56$ & $8.05$ & $\pm 0.17$ & \boldmath$3.26$ & \boldmath$\pm 0.08$ & $29.00$ & $\pm 0.00$ & \boldmath$20.84$ & \boldmath$\pm 0.00$ \\

\bottomrule
\end{tabular}}}

\caption{Training time, average test time per example, and model size for random and k-means trees.}
\label{tab:random-vs-kmeans-comp-perf}
\end{table}

==> tables/table-trees-maxleaves-logistic.tex <==

\begin{table}[H]
\centering
\footnotesize{
\resizebox{\textwidth}{!}{
\tabcolsep=5pt
\begin{tabular}{l|r@{}lr@{}lr@{}l|r@{}lr@{}lr@{}l}
\specialrule{0.94pt}{0.4ex}{0.65ex}
Pre-leaf degree & \multicolumn{2}{c}{25} & \multicolumn{2}{c}{100} & \multicolumn{2}{c|}{400} 
& \multicolumn{2}{c}{25} & \multicolumn{2}{c}{100} & \multicolumn{2}{c}{400} \\
\specialrule{0.94pt}{0.4ex}{0.65ex}
& \multicolumn{6}{c|}{$p@1$ [\%]}
& \multicolumn{6}{c}{$T/N_{\textrm{test}}$ [ms]} \\
\midrule
% \eurlex & \boldmath$80.62$ & \boldmath$\pm 0.12$ & $80.51$ & $\pm 0.16$ & $79.49$ & $\pm 0.39$ & \boldmath$0.15$ & \boldmath$\pm 0.00$ & $0.39$ & $\pm 0.03$ & $0.62$ & $\pm 0.02$ \\
% \amazoncatsmall & $93.05$ & $\pm 0.02$ & $93.04$ & $\pm 0.02$ & \boldmath$93.07$ & \boldmath$\pm 0.02$ & \boldmath$0.14$ & \boldmath$\pm 0.02$ & $0.32$ & $\pm 0.03$ & $0.67$ & $\pm 0.04$ \\
% \wikiten & $85.28$ & $\pm 0.08$ & $85.36$ & $\pm 0.09$ & \boldmath$85.41$ & \boldmath$\pm 0.06$ & \boldmath$2.07$ & \boldmath$\pm 0.30$ & $5.35$ & $\pm 0.32$ & $11.43$ & $\pm 0.21$ \\
% \deliciouslarge & $49.56$ & $\pm 0.03$ & $49.55$ & $\pm 0.05$ & \boldmath$49.62$ & \boldmath$\pm 0.03$ & \boldmath$6.25$ & \boldmath$\pm 0.35$ & $9.89$ & $\pm 0.89$ & $18.23$ & $\pm 0.72$ \\
\wikilshtc & $61.42$ & $\pm 0.03$ & $61.96$ & $\pm 0.03$ & \boldmath$62.16$ & \boldmath$\pm 0.05$ & \boldmath$0.66$ & \boldmath$\pm 0.04$ & $1.77$ & $\pm 0.11$ & $4.21$ & $\pm 0.10$ \\
\wikipedia & $65.72$ & $\pm 0.12$ & \boldmath$66.20$ & \boldmath$\pm 0.05$ & $65.95$ & $\pm 0.10$ & \boldmath$3.52$ & \boldmath$\pm 0.05$ & $6.67$ & $\pm 0.23$ & $20.13$ & $\pm 1.07$ \\
\amazon & $41.83$ & $\pm 0.02$ & \boldmath$43.54$ & \boldmath$\pm 0.01$ & $43.21$ & $\pm 0.03$ & \boldmath$1.61$ & \boldmath$\pm 0.04$ & $4.13$ & $\pm 0.28$ & $11.74$ & $\pm 0.46$ \\
\amazonlarge & $46.07$ & $\pm 0.01$ & $46.09$ & $\pm 0.02$ & \boldmath$46.13$ & \boldmath$\pm 0.01$ & \boldmath$1.47$ & \boldmath$\pm 0.00$ & $3.26$ & $\pm 0.08$ & $11.45$ & $\pm 0.22$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}
& \multicolumn{6}{c|}{$T_{\textrm{train}}$ [h]}
& \multicolumn{6}{c}{$M_{\textrm{size}}$ [GB]} \\
\midrule
% \eurlex & \boldmath$0.01$ & \boldmath$\pm 0.00$ & $0.02$ & $\pm 0.00$ & $0.04$ & $\pm 0.00$ & $0.03$ & $\pm 0.00$ & \boldmath$0.02$ & \boldmath$\pm 0.00$ & \boldmath$0.02$ & \boldmath$\pm 0.00$ \\
% \amazoncatsmall & \boldmath$0.36$ & \boldmath$\pm 0.03$ & $0.72$ & $\pm 0.02$ & $1.38$ & $\pm 0.03$ & $0.38$ & $\pm 0.00$ & $0.35$ & $\pm 0.00$ & \boldmath$0.34$ & \boldmath$\pm 0.00$ \\
% \wikiten & \boldmath$0.09$ & \boldmath$\pm 0.01$ & $0.21$ & $\pm 0.00$ & $0.32$ & $\pm 0.01$ & $0.73$ & $\pm 0.00$ & $0.58$ & $\pm 0.00$ & \boldmath$0.37$ & \boldmath$\pm 0.00$ \\
% \deliciouslarge & \boldmath$2.14$ & \boldmath$\pm 0.11$ & $2.58$ & $\pm 0.15$ & $4.18$ & $\pm 0.23$ & $1.14$ & $\pm 0.00$ & $0.95$ & $\pm 0.00$ & \boldmath$0.86$ & \boldmath$\pm 0.00$ \\
\wikilshtc & \boldmath$2.36$ & \boldmath$\pm 0.05$ & $2.95$ & $\pm 0.15$ & $4.83$ & $\pm 0.29$ & $3.28$ & $\pm 0.00$ & $2.73$ & $\pm 0.00$ & \boldmath$2.47$ & \boldmath$\pm 0.00$ \\
\wikipedia & \boldmath$12.40$ & \boldmath$\pm 0.08$ & $16.10$ & $\pm 0.44$ & $34.15$ & $\pm 0.46$ & $10.60$ & $\pm 0.01$ & $8.89$ & $\pm 0.00$ & \boldmath$7.94$ & \boldmath$\pm 0.00$ \\
\amazon & \boldmath$0.42$ & \boldmath$\pm 0.01$ & $0.56$ & $\pm 0.00$ & $1.01$ & $\pm 0.05$ & $2.20$ & $\pm 0.00$ & $2.26$ & $\pm 0.00$ & \boldmath$1.52$ & \boldmath$\pm 0.00$ \\
\amazonlarge & \boldmath$5.18$ & \boldmath$\pm 0.25$ & $7.07$ & $\pm 0.56$ & $16.41$ & $\pm 0.52$ & $24.00$ & $\pm 0.00$ & $20.84$ & $\pm 0.00$ & \boldmath$19.35$ & \boldmath$\pm 0.01$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}
\end{tabular}}}

\caption{Precision@1, average prediction time per example, training time and model size for $2$-means trees and degree of pre-leaves equal 25, 100, and 400 for logistic loss.}
\label{tab:k-means-tree-maxleaves-logistic}
\end{table}



==> tables/table-trees-maxleaves-sh.tex <==

\begin{table}[H]
\centering
\footnotesize{
\resizebox{\textwidth}{!}{
\tabcolsep=5pt
\begin{tabular}{l|r@{}lr@{}lr@{}l|r@{}lr@{}lr@{}l}
\specialrule{0.94pt}{0.4ex}{0.65ex}
Pre-leaf degree & \multicolumn{2}{c}{25} & \multicolumn{2}{c}{100} & \multicolumn{2}{c|}{400} 
& \multicolumn{2}{c}{25} & \multicolumn{2}{c}{100} & \multicolumn{2}{c}{400} \\
\specialrule{0.94pt}{0.4ex}{0.65ex}
& \multicolumn{6}{c|}{$p@1$ [\%]}
& \multicolumn{6}{c}{$T/N_{\textrm{test}}$ [ms]} \\
\midrule
% \eurlex & \boldmath$80.31$ & \boldmath$\pm 0.19$ & $80.17$ & $\pm 0.27$ & $79.21$ & $\pm 0.56$ & \boldmath$0.09$ & \boldmath$\pm 0.01$ & $0.24$ & $\pm 0.02$ & $0.54$ & $\pm 0.02$ \\
% \amazoncatsmall & $92.36$ & $\pm 0.04$ & $92.40$ & $\pm 0.04$ & \boldmath$92.53$ & \boldmath$\pm 0.08$ & \boldmath$0.12$ & \boldmath$\pm 0.02$ & $0.19$ & $\pm 0.00$ & $0.51$ & $\pm 0.06$ \\
% \wikiten & $83.72$ & $\pm 0.12$ & \boldmath$84.17$ & \boldmath$\pm 0.10$ & $83.90$ & $\pm 0.14$ & \boldmath$1.92$ & \boldmath$\pm 0.17$ & $2.87$ & $\pm 0.08$ & $6.46$ & $\pm 0.27$ \\
% \deliciouslarge & $46.24$ & $\pm 0.06$ & $46.30$ & $\pm 0.07$ & \boldmath$46.37$ & \boldmath$\pm 0.10$ & \boldmath$4.53$ & \boldmath$\pm 0.46$ & $10.07$ & $\pm 0.23$ & $17.12$ & $\pm 1.12$ \\
\wikilshtc & $61.96$ & $\pm 0.03$ & $62.78$ & $\pm 0.03$ & \boldmath$63.19$ & \boldmath$\pm 0.03$ & \boldmath$0.51$ & \boldmath$\pm 0.03$ & $0.86$ & $\pm 0.06$ & $1.78$ & $\pm 0.03$ \\
\wikipedia & $66.01$ & $\pm 0.10$ & $66.77$ & $\pm 0.08$ & \boldmath$66.90$ & \boldmath$\pm 0.06$ & \boldmath$2.29$ & \boldmath$\pm 0.03$ & $2.86$ & $\pm 0.07$ & $6.14$ & $\pm 0.11$ \\
\amazon & $42.93$ & $\pm 0.02$ & \boldmath$43.31$ & \boldmath$\pm 0.03$ & $43.25$ & $\pm 0.04$ & \boldmath$1.12$ & \boldmath$\pm 0.06$ & $1.32$ & $\pm 0.08$ & $2.43$ & $\pm 0.08$ \\
\amazonlarge & $45.84$ & $\pm 0.02$ & $46.23$ & $\pm 0.01$ & \boldmath$46.72$ & \boldmath$\pm 0.01$ & \boldmath$1.27$ & \boldmath$\pm 0.10$ & $1.96$ & $\pm 0.05$ & $5.61$ & $\pm 0.23$ \\


\specialrule{0.94pt}{0.4ex}{0.65ex}
& \multicolumn{6}{c|}{$T_{\textrm{train}}$ [h]}
& \multicolumn{6}{c}{$M_{\textrm{size}}$ [GB]} \\
\midrule
% \eurlex & \boldmath$0.00$ & \boldmath$\pm 0.00$ & $0.01$ & $\pm 0.00$ & $0.02$ & $\pm 0.00$ & \boldmath$0.00$ & \boldmath$\pm 0.00$ & $0.00$ & $\pm 0.00$ & $0.00$ & $\pm 0.00$ \\
% \amazoncatsmall & \boldmath$0.17$ & \boldmath$\pm 0.02$ & $0.29$ & $\pm 0.00$ & $0.70$ & $\pm 0.05$ & $0.21$ & $\pm 0.00$ & $0.19$ & $\pm 0.00$ & \boldmath$0.18$ & \boldmath$\pm 0.00$ \\
% \wikiten & \boldmath$0.10$ & \boldmath$\pm 0.00$ & $0.11$ & $\pm 0.00$ & $0.30$ & $\pm 0.02$ & $0.12$ & $\pm 0.00$ & \boldmath$0.06$ & \boldmath$\pm 0.00$ & $0.08$ & $\pm 0.00$ \\
% \deliciouslarge & \boldmath$3.08$ & \boldmath$\pm 0.13$ & $5.51$ & $\pm 0.29$ & $8.03$ & $\pm 0.57$ & $2.30$ & $\pm 0.00$ & $1.82$ & $\pm 0.00$ & \boldmath$1.56$ & \boldmath$\pm 0.00$ \\
\wikilshtc & \boldmath$1.54$ & \boldmath$\pm 0.03$ & $1.60$ & $\pm 0.06$ & $2.28$ & $\pm 0.10$ & $1.20$ & $\pm 0.00$ & $0.97$ & $\pm 0.00$ & \boldmath$0.84$ & \boldmath$\pm 0.00$ \\
\wikipedia & \boldmath$7.41$ & \boldmath$\pm 0.14$ & $9.48$ & $\pm 0.33$ & $19.32$ & $\pm 0.31$ & $2.23$ & $\pm 0.00$ & $1.78$ & $\pm 0.00$ & \boldmath$1.49$ & \boldmath$\pm 0.00$ \\
\amazon & \boldmath$0.39$ & \boldmath$\pm 0.01$ & $0.40$ & $\pm 0.01$ & $0.68$ & $\pm 0.02$ & $0.80$ & $\pm 0.00$ & $0.63$ & $\pm 0.00$ & \boldmath$0.51$ & \boldmath$\pm 0.00$ \\
\amazonlarge & \boldmath$4.80$ & \boldmath$\pm 0.29$ & $5.44$ & $\pm 0.13$ & $12.45$ & $\pm 0.74$ & $11.80$ & $\pm 0.00$ & $9.86$ & $\pm 0.00$ & \boldmath$8.60$ & \boldmath$\pm 0.00$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}
\end{tabular}}}

\caption{Precision@1, average prediction time per example, training time and model size for $2$-means trees, degree of pre-leaves equal 25, 100, and 400, and squared hinge loss.}
\label{tab:k-means-tree-maxleaves}
\end{table}



==> tables/table-trees-maxleaves.tex <==

\begin{table}[H]
\centering

\begin{subtable}{\textwidth}
\footnotesize{
\resizebox{\textwidth}{!}{
\tabcolsep=5pt
\begin{tabular}{l|r@{}lr@{}lr@{}l|r@{}lr@{}lr@{}l}
\specialrule{0.94pt}{0.4ex}{0.65ex}
Pre-leaf degree & \multicolumn{2}{c}{25} & \multicolumn{2}{c}{100} & \multicolumn{2}{c|}{400} 
& \multicolumn{2}{c}{25} & \multicolumn{2}{c}{100} & \multicolumn{2}{c}{400} \\
\specialrule{0.94pt}{0.4ex}{0.65ex}
& \multicolumn{6}{c|}{$p@1$ [\%]}
& \multicolumn{6}{c}{$T/N_{\textrm{test}}$ [ms]} \\
\midrule
% \eurlex & \boldmath$80.62$ & \boldmath$\pm 0.12$ & $80.51$ & $\pm 0.16$ & $79.49$ & $\pm 0.39$ & \boldmath$0.15$ & \boldmath$\pm 0.00$ & $0.39$ & $\pm 0.03$ & $0.62$ & $\pm 0.02$ \\
% \amazoncatsmall & $93.05$ & $\pm 0.02$ & $93.04$ & $\pm 0.02$ & \boldmath$93.07$ & \boldmath$\pm 0.02$ & \boldmath$0.14$ & \boldmath$\pm 0.02$ & $0.32$ & $\pm 0.03$ & $0.67$ & $\pm 0.04$ \\
% \wikiten & $85.28$ & $\pm 0.08$ & $85.36$ & $\pm 0.09$ & \boldmath$85.41$ & \boldmath$\pm 0.06$ & \boldmath$2.07$ & \boldmath$\pm 0.30$ & $5.35$ & $\pm 0.32$ & $11.43$ & $\pm 0.21$ \\
% \deliciouslarge & $49.56$ & $\pm 0.03$ & $49.55$ & $\pm 0.05$ & \boldmath$49.62$ & \boldmath$\pm 0.03$ & \boldmath$6.25$ & \boldmath$\pm 0.35$ & $9.89$ & $\pm 0.89$ & $18.23$ & $\pm 0.72$ \\
\wikilshtc & $61.42$ & $\pm 0.03$ & $61.96$ & $\pm 0.03$ & \boldmath$62.16$ & \boldmath$\pm 0.05$ & \boldmath$0.66$ & \boldmath$\pm 0.04$ & $1.77$ & $\pm 0.11$ & $4.21$ & $\pm 0.10$ \\
\wikipedia & $65.72$ & $\pm 0.12$ & \boldmath$66.20$ & \boldmath$\pm 0.05$ & $65.95$ & $\pm 0.10$ & \boldmath$3.52$ & \boldmath$\pm 0.05$ & $6.67$ & $\pm 0.23$ & $20.13$ & $\pm 1.07$ \\
\amazon & $41.83$ & $\pm 0.02$ & \boldmath$43.54$ & \boldmath$\pm 0.01$ & $43.21$ & $\pm 0.03$ & \boldmath$1.61$ & \boldmath$\pm 0.04$ & $4.13$ & $\pm 0.28$ & $11.74$ & $\pm 0.46$ \\
\amazonlarge & $46.07$ & $\pm 0.01$ & $46.09$ & $\pm 0.02$ & \boldmath$46.13$ & \boldmath$\pm 0.01$ & \boldmath$1.47$ & \boldmath$\pm 0.00$ & $3.26$ & $\pm 0.08$ & $11.45$ & $\pm 0.22$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}
& \multicolumn{6}{c|}{$T_{\textrm{train}}$ [h]}
& \multicolumn{6}{c}{$M_{\textrm{size}}$ [GB]} \\
\midrule
% \eurlex & \boldmath$0.01$ & \boldmath$\pm 0.00$ & $0.02$ & $\pm 0.00$ & $0.04$ & $\pm 0.00$ & $0.03$ & $\pm 0.00$ & \boldmath$0.02$ & \boldmath$\pm 0.00$ & \boldmath$0.02$ & \boldmath$\pm 0.00$ \\
% \amazoncatsmall & \boldmath$0.36$ & \boldmath$\pm 0.03$ & $0.72$ & $\pm 0.02$ & $1.38$ & $\pm 0.03$ & $0.38$ & $\pm 0.00$ & $0.35$ & $\pm 0.00$ & \boldmath$0.34$ & \boldmath$\pm 0.00$ \\
% \wikiten & \boldmath$0.09$ & \boldmath$\pm 0.01$ & $0.21$ & $\pm 0.00$ & $0.32$ & $\pm 0.01$ & $0.73$ & $\pm 0.00$ & $0.58$ & $\pm 0.00$ & \boldmath$0.37$ & \boldmath$\pm 0.00$ \\
% \deliciouslarge & \boldmath$2.14$ & \boldmath$\pm 0.11$ & $2.58$ & $\pm 0.15$ & $4.18$ & $\pm 0.23$ & $1.14$ & $\pm 0.00$ & $0.95$ & $\pm 0.00$ & \boldmath$0.86$ & \boldmath$\pm 0.00$ \\
\wikilshtc & \boldmath$2.36$ & \boldmath$\pm 0.05$ & $2.95$ & $\pm 0.15$ & $4.83$ & $\pm 0.29$ & $3.28$ & $\pm 0.00$ & $2.73$ & $\pm 0.00$ & \boldmath$2.47$ & \boldmath$\pm 0.00$ \\
\wikipedia & \boldmath$12.40$ & \boldmath$\pm 0.08$ & $16.10$ & $\pm 0.44$ & $34.15$ & $\pm 0.46$ & $10.60$ & $\pm 0.01$ & $8.89$ & $\pm 0.00$ & \boldmath$7.94$ & \boldmath$\pm 0.00$ \\
\amazon & \boldmath$0.42$ & \boldmath$\pm 0.01$ & $0.56$ & $\pm 0.00$ & $1.01$ & $\pm 0.05$ & $2.20$ & $\pm 0.00$ & $2.26$ & $\pm 0.00$ & \boldmath$1.52$ & \boldmath$\pm 0.00$ \\
\amazonlarge & \boldmath$5.18$ & \boldmath$\pm 0.25$ & $7.07$ & $\pm 0.56$ & $16.41$ & $\pm 0.52$ & $24.00$ & $\pm 0.00$ & $20.84$ & $\pm 0.00$ & \boldmath$19.35$ & \boldmath$\pm 0.01$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}
\end{tabular}}}
\caption{Results for logistic loss.}
\end{subtable}

\vspace{12pt}

\begin{subtable}{\textwidth}
\footnotesize{
\resizebox{\textwidth}{!}{
\tabcolsep=5pt
\begin{tabular}{l|r@{}lr@{}lr@{}l|r@{}lr@{}lr@{}l}
\specialrule{0.94pt}{0.4ex}{0.65ex}
Pre-leaf degree & \multicolumn{2}{c}{25} & \multicolumn{2}{c}{100} & \multicolumn{2}{c|}{400} 
& \multicolumn{2}{c}{25} & \multicolumn{2}{c}{100} & \multicolumn{2}{c}{400} \\
\specialrule{0.94pt}{0.4ex}{0.65ex}
& \multicolumn{6}{c|}{$p@1$ [\%]}
& \multicolumn{6}{c}{$T/N_{\textrm{test}}$ [ms]} \\
\midrule
% \eurlex & \boldmath$80.31$ & \boldmath$\pm 0.19$ & $80.17$ & $\pm 0.27$ & $79.21$ & $\pm 0.56$ & \boldmath$0.09$ & \boldmath$\pm 0.01$ & $0.24$ & $\pm 0.02$ & $0.54$ & $\pm 0.02$ \\
% \amazoncatsmall & $92.36$ & $\pm 0.04$ & $92.40$ & $\pm 0.04$ & \boldmath$92.53$ & \boldmath$\pm 0.08$ & \boldmath$0.12$ & \boldmath$\pm 0.02$ & $0.19$ & $\pm 0.00$ & $0.51$ & $\pm 0.06$ \\
% \wikiten & $83.72$ & $\pm 0.12$ & \boldmath$84.17$ & \boldmath$\pm 0.10$ & $83.90$ & $\pm 0.14$ & \boldmath$1.92$ & \boldmath$\pm 0.17$ & $2.87$ & $\pm 0.08$ & $6.46$ & $\pm 0.27$ \\
% \deliciouslarge & $46.24$ & $\pm 0.06$ & $46.30$ & $\pm 0.07$ & \boldmath$46.37$ & \boldmath$\pm 0.10$ & \boldmath$4.53$ & \boldmath$\pm 0.46$ & $10.07$ & $\pm 0.23$ & $17.12$ & $\pm 1.12$ \\
\wikilshtc & $61.96$ & $\pm 0.03$ & $62.78$ & $\pm 0.03$ & \boldmath$63.19$ & \boldmath$\pm 0.03$ & \boldmath$0.51$ & \boldmath$\pm 0.03$ & $0.86$ & $\pm 0.06$ & $1.78$ & $\pm 0.03$ \\
\wikipedia & $66.01$ & $\pm 0.10$ & $66.77$ & $\pm 0.08$ & \boldmath$66.90$ & \boldmath$\pm 0.06$ & \boldmath$2.29$ & \boldmath$\pm 0.03$ & $2.86$ & $\pm 0.07$ & $6.14$ & $\pm 0.11$ \\
\amazon & $42.93$ & $\pm 0.02$ & \boldmath$43.31$ & \boldmath$\pm 0.03$ & $43.25$ & $\pm 0.04$ & \boldmath$1.12$ & \boldmath$\pm 0.06$ & $1.32$ & $\pm 0.08$ & $2.43$ & $\pm 0.08$ \\
\amazonlarge & $45.84$ & $\pm 0.02$ & $46.23$ & $\pm 0.01$ & \boldmath$46.72$ & \boldmath$\pm 0.01$ & \boldmath$1.27$ & \boldmath$\pm 0.10$ & $1.96$ & $\pm 0.05$ & $5.61$ & $\pm 0.23$ \\


\specialrule{0.94pt}{0.4ex}{0.65ex}
& \multicolumn{6}{c|}{$T_{\textrm{train}}$ [h]}
& \multicolumn{6}{c}{$M_{\textrm{size}}$ [GB]} \\
\midrule
% \eurlex & \boldmath$0.00$ & \boldmath$\pm 0.00$ & $0.01$ & $\pm 0.00$ & $0.02$ & $\pm 0.00$ & \boldmath$0.00$ & \boldmath$\pm 0.00$ & $0.00$ & $\pm 0.00$ & $0.00$ & $\pm 0.00$ \\
% \amazoncatsmall & \boldmath$0.17$ & \boldmath$\pm 0.02$ & $0.29$ & $\pm 0.00$ & $0.70$ & $\pm 0.05$ & $0.21$ & $\pm 0.00$ & $0.19$ & $\pm 0.00$ & \boldmath$0.18$ & \boldmath$\pm 0.00$ \\
% \wikiten & \boldmath$0.10$ & \boldmath$\pm 0.00$ & $0.11$ & $\pm 0.00$ & $0.30$ & $\pm 0.02$ & $0.12$ & $\pm 0.00$ & \boldmath$0.06$ & \boldmath$\pm 0.00$ & $0.08$ & $\pm 0.00$ \\
% \deliciouslarge & \boldmath$3.08$ & \boldmath$\pm 0.13$ & $5.51$ & $\pm 0.29$ & $8.03$ & $\pm 0.57$ & $2.30$ & $\pm 0.00$ & $1.82$ & $\pm 0.00$ & \boldmath$1.56$ & \boldmath$\pm 0.00$ \\
\wikilshtc & \boldmath$1.54$ & \boldmath$\pm 0.03$ & $1.60$ & $\pm 0.06$ & $2.28$ & $\pm 0.10$ & $1.20$ & $\pm 0.00$ & $0.97$ & $\pm 0.00$ & \boldmath$0.84$ & \boldmath$\pm 0.00$ \\
\wikipedia & \boldmath$7.41$ & \boldmath$\pm 0.14$ & $9.48$ & $\pm 0.33$ & $19.32$ & $\pm 0.31$ & $2.23$ & $\pm 0.00$ & $1.78$ & $\pm 0.00$ & \boldmath$1.49$ & \boldmath$\pm 0.00$ \\
\amazon & \boldmath$0.39$ & \boldmath$\pm 0.01$ & $0.40$ & $\pm 0.01$ & $0.68$ & $\pm 0.02$ & $0.80$ & $\pm 0.00$ & $0.63$ & $\pm 0.00$ & \boldmath$0.51$ & \boldmath$\pm 0.00$ \\
\amazonlarge & \boldmath$4.80$ & \boldmath$\pm 0.29$ & $5.44$ & $\pm 0.13$ & $12.45$ & $\pm 0.74$ & $11.80$ & $\pm 0.00$ & $9.86$ & $\pm 0.00$ & \boldmath$8.60$ & \boldmath$\pm 0.00$ \\

\specialrule{0.94pt}{0.4ex}{0.65ex}
\end{tabular}}}
\caption{Results for squared hinge loss.}
\end{subtable}

\caption{Precision@1, average prediction time per example, training time and model size for $2$-means trees and degree of pre-leaves equal 25, 100, and 400.}
\label{tab:k-means-tree-maxleaves}
\end{table}


